Are Decoder-Only Large Language Models the Silver Bullet for Code Search?

Code search is essential for code reuse, allowing developers to efficiently locate relevant code snippets. The advent of powerful decoder-only Large Language Models (LLMs) has revolutionized many code intelligence tasks. However, their effectiveness for the retrieval-based task of code search, particularly compared to established encoder-based models, remains underexplored. This paper addresses this gap by presenting a large-scale systematic evaluation of eleven decoder-only LLMs, analyzing their performance across zero-shot and fine-tuned settings. Our results show that fine-tuned decoder-only models, particularly CodeGemma, significantly outperform encoder-only models like UniXcoder, achieving a 40.4% higher Mean Average Precision (MAP) on the CoSQA$^+$ benchmark. Our analysis further reveals two crucial nuances for practitioners: first, the relationship between model size and performance is non-monotonic, with mid-sized models often outperforming larger variants; second, the composition of the training data is critical, as a multilingual dataset enhances generalization while a small amount of data from a specific language can act as noise and interfere with model effectiveness. These findings offer a comprehensive guide to selecting and optimizing modern LLMs for code search.

==> figures/fig_pca.tex <==
\begin{figure*}[t]
    \centering
    \subfloat[\scriptsize \revised{UniXcoder Embedding Space Before Fine-tuning}]{
    \includegraphics[width=0.44\textwidth]{figures/figure_pca_before_finetuning_random.pdf}
    \label{fig:pca_before_finetuning_random}
    }
    % \quad
    \hspace{0.3em}  
    \subfloat[\scriptsize \revised{UniXcoder Embedding Space After Fine-tuning}]{
    \includegraphics[width=0.44\textwidth]{figures/figure_pca_after_finetuning_random.pdf}
    \label{fig:pca_after_finetuning_random}}
    % \quad

    \vspace{0pt} 
    \centering
    \caption{\revised{PCA Visualization of UniXcoder's Embedding Space Before and After Fine-tuning on CSN.}}
    \label{fig:unixicoder_PCA}
\end{figure*}

==> figures/fig_pca_codegemma.tex <==
\begin{figure*}[t]
    \centering
    \subfloat[\scriptsize \revised{CodeGemma Embedding Space Before Fine-tuning}]{
    \includegraphics[width=0.44\textwidth]{figures/figure_pca_before_finetuning_random_CodeGemma.pdf}
    \label{fig:pca_before_finetuning_random_CodeGemma}
    }
    % \quad
    \hspace{0.3em}  % 控制水平间距
    \subfloat[\scriptsize \revised{CodeGemma Embedding Space After Fine-tuning}]{
    \includegraphics[width=0.44\textwidth]{figures/figure_pca_after_finetuning_random_CodeGemma.pdf}
    \label{fig:pca_after_finetuning_random_CodeGemma}}
    % \quad

    \vspace{0pt} 
    \centering
    \caption{\revised{PCA Visualization of CodeGemma's Embedding Space Before and After Fine-tuning on CSN.}}
    \label{fig:CodeGemma_pca}
\end{figure*}

==> figures/overview.tex <==
\begin{figure}[htb]
	\centering
        \vspace{-3mm}
	\includegraphics[width=0.82\columnwidth]{pics/method_overview}
        \vspace{-2mm}

	\caption{Overview of Interactive Methodology for Crash Bug Resolution with LLMs}
	\label{fig:overview}
    \vspace{-3mm}
\end{figure}

==> figures/sing_language.tex <==
\begin{figure*}[t]
    \centering
    % Subfigure for the CSN Benchmark results
    \subfloat[\revised{Performance on the CSN Benchmark}]{
        \includegraphics[width=0.48\textwidth]{figures/Single_lang_finetune_performance_csn.pdf}
        \label{fig:Single_lang_finetune_performance_csn}
    }
    \hspace{0.3em} % Controls the horizontal space between figures
    % Subfigure for the CoSQA+ Benchmark results
    \subfloat[\revised{Performance on the CoSQA+ Benchmark}]{
        \includegraphics[width=0.48\textwidth]{figures/Single_lang_finetune_performance_COSQA_map.pdf}
        \label{fig:Single_lang_finetune_performance_COSQA_map}
    }
    % Main caption for the entire figure
    \caption{
            \revised{Single-Language Fine-Tuning on Model Performance.}
    }
    \label{fig:single_language_fine_tuning_results}
\end{figure*}



==> figures/single_language_step.tex <==
\begin{figure}[t]
    \centering
    \centering
   \begin{minipage}[b]{.48\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/CodeGemma_single_lang_finetune_steps_CSN.pdf}
        \vspace{-20pt} 
        \caption{\revised{Training Curves for CodeGemma on the CSN Benchmark.}}
        \label{fig:CodeGemma_single_lang_finetune_steps_CSN}
    \end{minipage}\quad
    \begin{minipage}[b]{.48\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/CodeGemma_single_lang_finetune_steps_COSQA_MAP.pdf}
        \vspace{-20pt} 
        \caption{\revised{Training Curves for CodeGemma on the CoSQA+ Benchmark.}}
        \label{fig:CodeGemma_single_lang_finetune_steps_COSQA_MAP}
    \end{minipage}
\end{figure}



==> reference_old.tex <==
@article{arslan2024survey,
  title={A Survey on RAG with LLMs},
  author={Arslan, Muhammad and Ghanem, Hussam and Munawar, Saba and Cruz, Christophe},
  journal={Procedia computer science},
  volume={246},
  pages={3781--3790},
  year={2024},\section{discussion}
\revRtwo{In the session, we discuss some practical implications for researchers and developers. In addition, we discuss potential research directions for future work.}

% \revised{In **this section**, we discuss **the** practical implications for researchers and developers. Furthermore, we discuss potential research **directions** for future work.}
% ^-- MODIFIED: "session" -> "this section", added "the", "direction" -> "directions"

\subsection{\revised{Practical Implications}}

\revised{Based on our systematic evaluation, we offer the following recommendations for those looking to apply language models to code search tasks:}

\revised{\textbf{For Zero-Shot Scenarios}: When fine-tuning is not feasible due to resource or time constraints, we recommend using specialized encoder-only models like UniXcoder. Despite its smaller size, it offers a competitive balance of performance and efficiency, outperforming many recent, larger decoder-only LLMs in zero-shot settings.}

% \revised{\textbf{For Fine-Tuning Scenarios}: If resources for fine-tuning are available, we strongly recommend decoder-only LLMs, particularly models from the Gemma \revRtwo{and Qwen2.5-Coder} family. Our results show that its architecture demonstrates superior understanding and generalization capabilities after fine-tuning, surpassing even more recent and larger models.}
\revised{\textbf{For Fine-Tuning Scenarios}: If resources for fine-tuning are available, we strongly recommend decoder-only LLMs, particularly models from the Gemma \revRtwo{and Qwen2.5-Coder} \revRtwo{families}. Our results show that \revRtwo{their architectures demonstrate} superior understanding and generalization capabilities after fine-tuning, surpassing even \revRtwo{other} recent and larger models.}

\revised{\textbf{For Fine-tuning Method}: We recommend using supervised contrastive learning (SupCon). This method is highly effective at improving a model's ability to distinguish between relevant and irrelevant code snippets, which is the core of the code search task.}

\revised{\textbf{For Training Data:} Fine-tuning on a specialized code search dataset yields statistically significant improvements over using a general-purpose information retrieval dataset. Training on a multilingual dataset can bring stronger generalization ability and more stable performance compared to using a single-language dataset. Meanwhile, the data composition is critical, as a small amount of data from a specific language may interfere with the model's training effectiveness, potentially acting as statistical noise.}

\revised{\textbf{For Model \revRtwo{Size}}: Model size is not always proportional to performance. Our experiments indicate that a larger model does not guarantee better results for code search. We \revRtwo{observe} a non-monotonic trend where a mid-sized model (e.g., 1.5B) sometimes outperforms its larger counterparts. This suggests that practitioners may find a better cost-performance balance with moderately-sized models, but should determine the optimal size through targeted experiments.}

\revised{\textbf{For Resource Trade-offs:} The cost of fine-tuning should be justified. While the offline cost of fine-tuning a large model is significant, it is a one-time investment that can yield a substantial and lasting improvement in the final system's performance.}


\subsection{Future Work}\label{futureWork}

\revRtwo{Our findings not only provide practical guidance but also open up several avenues for future research:}

\begin{itemize} 
\item \revRtwo{\textbf{Developing Next-Generation Code Search Datasets:} Our study confirms that fine-tuning on specialized code search data (like CSN, which uses code comments as queries) yields superior results compared to general-purpose text. However, the nature of code search is evolving. Modern applications, such as RAG and AI agents, will generate queries that are far more diverse than traditional human-authored comments. This indicates a critical need for new, high-quality, and varied fine-tuning datasets that reflect both complex human intent and AI-generated retrieval queries.}

\item \revRtwo{\textbf{Accelerating Fine-Tuning without Performance Loss:} Although the current cost of full fine-tuning is a one-time investment, it remains substantial. For decoder-only LLMs, increasing the fine-tuning speed while ensuring no degradation in performance would significantly enhance their practical appeal. Future work should systematically evaluate the trade-offs of PEFT methods specifically for the code search task, aiming to optimize both training efficiency and final retrieval accuracy.}

\item \revRtwo{\textbf{Investigating the Non-Monotonic Scaling Effect:} Our discovery that model size does not monotonically improve performance (with a 1.5B parameter model outperforming larger counterparts) warrants deeper investigation. Future research should explore why this occurs. Is it due to optimization difficulties, the nature of the code search task, or catastrophic forgetting during fine-tuning? Identifying the ``sweet spot" for model scale in code search could lead to more efficient and effective models.}

\item \revRtwo{\textbf{Optimizing Data Composition:} We note that small amounts of data from specific languages might act as ``statistical noise" and hinder training. Future work could quantify this effect more precisely. What is the minimum data threshold required for a language to contribute positively to a multilingual model? Can curriculum learning or data re-weighting schemes mitigate the negative impact of low-resource languages in a multilingual dataset?}

\end{itemize}

% \begin{itemize}
% \item \revRtwo{\textbf{Developing Next-Generation Code Search Datasets:} Our study **confirms** that fine-tuning on specialized code search data (like CSN, which uses code comments as queries) **yields** superior results compared to general-purpose text. However, the nature of code search is evolving. Modern applications, such as RAG and AI agents, will generate queries that are far more diverse than traditional human-authored comments. This indicates a critical need for new, high-quality, and varied fine-tuning datasets that reflect both complex human intent and AI-generated retrieval queries.}

% \item \revRtwo{\textbf{Accelerating Fine-Tuning without Performance Loss:} Although the current cost of full fine-tuning is a one-time investment, it remains substantial. For decoder-only LLMs, increasing the fine-tuning speed while ensuring no degradation in performance would significantly enhance their practical appeal. Future work should systematically evaluate the trade-offs of PEFT methods specifically for the code search task, aiming to optimize both training efficiency and final retrieval accuracy.}

% \item \revRtwo{\textbf{Investigating the Non-Monotonic Scaling Effect:} Our discovery that model size does not monotonically improve performance (with a 1.5B parameter model outperforming larger counterparts) warrants deeper investigation. Future research should explore why this occurs. Is it due to optimization difficulties, the nature of the code search task, or catastrophic forgetting during fine-tuning? Identifying the ``sweet spot" for model scale in code search could lead to more efficient and effective models.}

% \item \revRtwo{\textbf{Optimizing Data Composition:} We **note** that small amounts of data from specific languages might act as ``statistical noise" and hinder training. Future work could quantify this effect more precisely. What is the minimum data threshold required for a language to contribute positively to a multilingual model? Can curriculum learning or data re-weighting schemes mitigate the negative impact of low-resource languages in a multilingual dataset?}
% \end{itemize}

  publisher={Elsevier}
}
@inproceedings{wang2025rag,
  title={Rag or fine-tuning? a comparative study on lcms-based code completion in industry},
  author={Wang, Chaozheng and Yang, Zezhou and Gao, Shuzheng and Gao, Cuiyun and Peng, Ting and Huang, Hailiang and Deng, Yuetang and Lyu, Michael},
  booktitle={Proceedings of the 33rd ACM International Conference on the Foundations of Software Engineering},
  pages={93--104},
  year={2025}
}
@article{du2024vul,
  title={Vul-rag: Enhancing llm-based vulnerability detection via knowledge-level rag},
  author={Du, Xueying and Zheng, Geng and Wang, Kaixin and Zou, Yi and Wang, Yujia and Deng, Wentai and Feng, Jiayi and Liu, Mingwei and Chen, Bihuan and Peng, Xin and others},
  journal={arXiv preprint arXiv:2406.11147},
  year={2024}
}

@article{gu2025retrieve,
  title={What to Retrieve for Effective Retrieval-Augmented Code Generation? An Empirical Study and Beyond},
  author={Gu, Wenchao and Chen, Juntao and Wang, Yanlin and Jiang, Tianyue and Li, Xingzhe and Liu, Mingwei and Liu, Xilin and Ma, Yuchi and Zheng, Zibin},
  journal={arXiv preprint arXiv:2503.20589},
  year={2025}
}

@inproceedings{feng2025learning,
  title={Learning to Look at the Other Side: A Semantic Probing Study of Word Embeddings in LLMs with Enabled Bidirectional Attention},
  author={Feng, Zhaoxin and Ma, Jianfei and Chersoni, Emmanuele and Zhao, Xiaojing and Bao, Xiaoyi},
  booktitle={Proceedings of the Annual Meeting of the Association for Computational Linguistics: ACL 2025},
  year={2025},
  organization={Association for Computational Linguistics}
}


@inproceedings{xu2024wizardlm,
  title={WizardLM: Empowering large pre-trained language models to follow complex instructions},
  author={Xu, Can and Sun, Qingfeng and Zheng, Kai and Geng, Xiubo and Zhao, Pu and Feng, Jiazhan and Tao, Chongyang and Lin, Qingwei and Jiang, Daxin},
  booktitle={The Twelfth International Conference on Learning Representations},
  year={2024}
}
@article{grattafiori2024llama,
  title={The llama 3 herd of models},
  author={Grattafiori, Aaron and Dubey, Abhimanyu and Jauhri, Abhinav and Pandey, Abhinav and Kadian, Abhishek and Al-Dahle, Ahmad and Letman, Aiesha and Mathur, Akhil and Schelten, Alan and Vaughan, Alex and others},
  journal={arXiv preprint arXiv:2407.21783},
  year={2024}
}
    @article{team2024codegemma,
  title={Codegemma: Open code models based on gemma},
  author={Team, CodeGemma and Zhao, Heri and Hui, Jeffrey and Howland, Joshua and Nguyen, Nam and Zuo, Siqi and Hu, Andrea and Choquette-Choo, Christopher A and Shen, Jingyue and Kelley, Joe and others},
  journal={arXiv preprint arXiv:2406.11409},
  year={2024}
}
@article{roziere2023code,
  title={Code llama: Open foundation models for code},
  author={Roziere, Baptiste and Gehring, Jonas and Gloeckle, Fabian and Sootla, Sten and Gat, Itai and Tan, Xiaoqing Ellen and Adi, Yossi and Liu, Jingyu and Sauvestre, Romain and Remez, Tal and others},
  journal={arXiv preprint arXiv:2308.12950},
  year={2023}
}




@misc{ChenyxEugene_DecoderLLMs_CodeSearch_2025,
  author       = {Chen, Yuxuan},
  title        = {DecoderLLMs-CodeSearch: Replication Package},
  year         = {2025},
  publisher    = {GitHub},
  howpublished = {\url{https://github.com/ChenyxEugene/DecoderLLMs-CodeSearch}},
  note         = {Accessed: November 2, 2025.}
}
@misc{SYSUSELab_HF_Collection_2025,
  author       = {{SYSUSELab}},
  title        = {Are Decoder-Only LLMs the Silver Bullet? (Collection)},
  year         = {2025},
  publisher    = {Hugging Face},
  journal      = {Hugging Face repository},
  howpublished = {\url{https://huggingface.co/collections/SYSUSELab/are-decoder-only-llms-the-silver-bullet}},
  note         = {Accessed: November 2, 2025.}
}

@misc{uukuguy_speechless_2024,
  author       = {uukuguy},
  title        = {speechless-code-mistral-7b-v1.0},
  year         = {2024},
  publisher    = {Hugging Face},
  journal      = {Hugging Face repository},
  howpublished = {\url{https://huggingface.co/uukuguy/speechless-code-mistral-7b-v1.0}}
}

@article{tao2024llms,
  title={Llms are also effective embedding models: An in-depth overview},
  author={Tao, Chongyang and Shen, Tao and Gao, Shen and Zhang, Junshuo and Li, Zhen and Hua, Kai and Hu, Wenpeng and Tao, Zhengwei and Ma, Shuai},
  journal={arXiv preprint arXiv:2412.12591},
  year={2024}
}

@article{behnamghader2025exploiting,
  title={Exploiting Instruction-Following Retrievers for Malicious Information Retrieval},
  author={BehnamGhader, Parishad and Meade, Nicholas and Reddy, Siva},
  journal={arXiv preprint arXiv:2503.08644},
  year={2025}
}

@inproceedings{yu2025gar,
  title={CA-GAR: Context-Aware Alignment of LLM Generation for Document Retrieval},
  author={Yu, Heng and Kang, Junfeng and Li, Rui and Liu, Qi and He, Liyang and Huang, Zhenya and Shen, Shuanghong and Lu, Junyu},
  booktitle={Findings of the Association for Computational Linguistics: ACL 2025},
  pages={5836--5849},
  year={2025}
}

@inproceedings{zhuang2024setwise,
  title={A setwise approach for effective and highly efficient zero-shot ranking with large language models},
  author={Zhuang, Shengyao and Zhuang, Honglei and Koopman, Bevan and Zuccon, Guido},
  booktitle={Proceedings of the 47th International ACM SIGIR Conference on Research and Development in Information Retrieval},
  pages={38--47},
  year={2024}
}

@inproceedings{he2025llm2rec,
  title={Llm2rec: Large language models are powerful embedding models for sequential recommendation},
  author={He, Yingzhi and Liu, Xiaohao and Zhang, An and Ma, Yunshan and Chua, Tat-Seng},
  booktitle={Proceedings of the 31st ACM SIGKDD Conference on Knowledge Discovery and Data Mining V. 2},
  pages={896--907},
  year={2025}
}

@inproceedings{wang2025pre,
  title={Pre-train, Align, and Disentangle: Empowering Sequential Recommendation with Large Language Models},
  author={Wang, Yuhao and Pan, Junwei and Jia, Pengyue and Wang, Wanyu and Wang, Maolin and Feng, Zhixiang and Li, Xiaotian and Jiang, Jie and Zhao, Xiangyu},
  booktitle={Proceedings of the 48th International ACM SIGIR Conference on Research and Development in Information Retrieval},
  pages={1455--1465},
  year={2025}
}

@inproceedings{man2025lusifer,
  title={LUSIFER: Language Universal Space Integration for Enhanced Representation in Multilingual Text Embedding Models},
  author={Man, Hieu and Ngo, Nghia Trung and Dac Lai, Viet and Rossi, Ryan A and Dernoncourt, Franck and Huu Nguyen, Thien},
  booktitle={Proceedings of the 48th International ACM SIGIR Conference on Research and Development in Information Retrieval},
  pages={1360--1370},
  year={2025}
}

@inproceedings{zeng2025scaling,
  title={Scaling sparse and dense retrieval in decoder-only llms},
  author={Zeng, Hansi and Killingback, Julian and Zamani, Hamed},
  booktitle={Proceedings of the 48th International ACM SIGIR Conference on Research and Development in Information Retrieval},
  pages={2679--2684},
  year={2025}
}


@misc{Qwen2.5-Coder-7B-Instruct,
  author       = {{Qwen Team}},
  title        = {Qwen2.5-Coder-7B-Instruct},
  year         = {2025},
  howpublished = {\url{https://huggingface.co/Qwen/Qwen2.5-Coder-7B-Instruct}},
  note         = {Accessed: 2025-07-04}
}

@misc{StarCoder2-7B,
  author       = {{BigCode Team}},
  title        = {StarCoder2-7B},
  year         = {2024},
  howpublished = {\url{https://huggingface.co/bigcode/starcoder2-7b}},
  note         = {Accessed: 2025-07-04}
}

@misc{ShearedLLaMA1.3B_HF,
  author       = {Princeton NLP},
  title        = {Sheared-LLaMA-1.3B Model Card},
  year         = {2023},
  howpublished = {\url{https://huggingface.co/princeton-nlp/Sheared-LLaMA-1.3B}},
  note         = {Accessed: 2025-08-20}
}

@misc{Llama2_7B_HF,
  author       = {Meta},
  title        = {Llama-2-7b-hf Model Card},
  year         = {2023},
  howpublished = {\url{https://huggingface.co/meta-llama/Llama-2-7b-hf}},
  note         = {Accessed: 2025-08-20}
}

@misc{Llama2_13B_HF,
  author       = {Meta},
  title        = {Llama-2-13b-hf Model Card},
  year         = {2023},
  howpublished = {\url{https://huggingface.co/meta-llama/Llama-2-13b-hf}},
  note         = {Accessed: 2025-08-20}
}

@misc{Qwen2_5_0.5B_HF,
  author       = {Qwen Team},
  title        = {Qwen2.5-Coder-0.5B-Instruct Model Card},
  year         = {2024},
  howpublished = {\url{https://huggingface.co/Qwen/Qwen2.5-Coder-0.5B-Instruct}},
  note         = {Accessed: 2025-08-20}
}

@misc{Qwen2_5_1.5B_HF,
  author       = {Qwen Team},
  title        = {Qwen2.5-Coder-1.5B-Instruct Model Card},
  year         = {2024},
  howpublished = {\url{https://huggingface.co/Qwen/Qwen2.5-Coder-1.5B-Instruct}},
  note         = {Accessed: 2025-08-20}
}

@misc{Qwen2_5_3B_HF,
  author       = {Qwen Team},
  title        = {Qwen2.5-Coder-3B-Instruct Model Card},
  year         = {2024},
  howpublished = {\url{https://huggingface.co/Qwen/Qwen2.5-Coder-3B-Instruct}},
  note         = {Accessed: 2025-08-20}
}

@misc{Qwen2_5_7B_HF,
  author       = {Qwen Team},
  title        = {Qwen2.5-Coder-7B-Instruct Model Card},
  year         = {2024},
  howpublished = {\url{https://huggingface.co/Qwen/Qwen2.5-Coder-7B- Instruct}},
  note         = {Accessed: 2025-08-20}
}

@misc{Qwen2_5_14B_HF,
  author       = {Qwen Team},
  title        = {Qwen2.5-Coder-14B-Instruct Model Card},
  year         = {2024},
  howpublished = {\url{https://huggingface.co/Qwen/Qwen2.5-Coder-14B-Instruct}},
  note         = {Accessed: 2025-08-20}
}
@misc{uukuguy2023speechless,
  author       = {uukuguy},
  title        = {speechless-code-mistral-7b-v1.0},
  howpublished = {\url{https://huggingface.co/uukuguy/speechless-code-mistral-7b-v1.0}},
  year         = {2023},
  note         = {Accessed: November 6, 2025.}
}

@article{lee2023platypus,
  title={Platypus: Quick, cheap, and powerful refinement of llms},
  author={Lee, Ariel N and Hunter, Cole J and Ruiz, Nataniel},
  journal={arXiv preprint arXiv:2308.07317},
  year={2023}
}
@misc{Lian2023OpenOrca,
  author       = {Lian, Wing and Goodson, B. and Pentland, E. and Cook, A. and Vong, C. and Teknium},
  title        = {OpenOrca: An open dataset of gpt augmented flan reasoning traces},
  howpublished = {\url{https://huggingface.co/datasets/Open-Orca/OpenOrca}},
  year         = {2023},
  note         = {Accessed: November 6, 2025.}
}

@article{brown2020language,
  title={Language models are few-shot learners},
  author={Brown, Tom and Mann, Benjamin and Ryder, Nick and Subbiah, Melanie and Kaplan, Jared D and Dhariwal, Prafulla and Neelakantan, Arvind and Shyam, Pranav and Sastry, Girish and Askell, Amanda and others},
  journal={Advances in neural information processing systems},
  volume={33},
  pages={1877--1901},
  year={2020}
}


@misc{Qwen2.5-Coder-Collection,
  author       = {Qwen Team},
  title        = {Qwen2.5-Coder},
  howpublished = {\url{https://huggingface.co/collections/Qwen/qwen25-coder}},
  month        = nov,
  year         = 2025,
  note         = {Accessed: November 6, 2025.}
}
@inproceedings{bui2021self,
  title={Self-supervised contrastive learning for code retrieval and summarization via semantic-preserving transformations},
  author={Bui, Nghi DQ and Yu, Yijun and Jiang, Lingxiao},
  booktitle={Proceedings of the 44th International ACM SIGIR Conference on Research and Development in Information Retrieval},
  pages={511--521},
  year={2021}
}



@misc{decoder2024,
  author = {Anonymous},
  title = {Decoder-Only Code Search},
  year = {2024},
  howpublished = {\url{https://anonymous.4open.science/r/decoder-only-code-search-82CD}},
  note = {Anonymous GitHub Repository}
}
@misc{mteb_leaderboard,
  author       = {{MTEB}},
  title        = {{MTEB Leaderboard}},
  year         = {2025},
  howpublished = {\url{https://huggingface.co/spaces/mteb/leaderboard}},
  note         = {Accessed: November 2, 2025.}
}

@inproceedings{sun2022importance,
  title={On the importance of building high-quality training datasets for neural code search},
  author={Sun, Zhensu and Li, Li and Liu, Yan and Du, Xiaoning and Li, Li},
  booktitle={Proceedings of the 44th International Conference on Software Engineering},
  pages={1609--1620},
  year={2022}
}

@inproceedings{icse2023ptmcomp,
  author       = {Changan Niu and
                  Chuanyi Li and
                  Vincent Ng and
                  Dongxiao Chen and
                  Jidong Ge and
                  Bin Luo},
  title        = {An Empirical Comparison of Pre-Trained Models of Source Code},
  booktitle    = {45th {IEEE/ACM} International Conference on Software Engineering,
                  {ICSE} 2023, Melbourne, Australia, May 14-20, 2023},
  pages        = {2136--2148},
  publisher    = {{IEEE}},
  year         = {2023},
  url          = {https://doi.org/10.1109/ICSE48619.2023.00180},
  doi          = {10.1109/ICSE48619.2023.00180},
  timestamp    = {Sun, 19 Jan 2025 13:14:58 +0100},
  biburl       = {https://dblp.org/rec/conf/icse/NiuLNCGL23.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{lozhkov2024starcoder,
  title={Starcoder 2 and the stack v2: The next generation},
  author={Lozhkov, Anton and Li, Raymond and Allal, Loubna Ben and Cassano, Federico and Lamy-Poirier, Joel and Tazi, Nouamane and Tang, Ao and Pykhtar, Dmytro and Liu, Jiawei and Wei, Yuxiang and others},
  journal={arXiv preprint arXiv:2402.19173},
  year={2024}
}

@article{hui2024qwen2,
  title={Qwen2. 5-coder technical report},
  author={Hui, Binyuan and Yang, Jian and Cui, Zeyu and Yang, Jiaxi and Liu, Dayiheng and Zhang, Lei and Liu, Tianyu and Zhang, Jiajun and Yu, Bowen and Lu, Keming and others},
  journal={arXiv preprint arXiv:2409.12186},
  year={2024}
}
@inproceedings{zhu2020ocor,
  title={OCoR: An overlapping-aware code retriever},
  author={Zhu, Qihao and Sun, Zeyu and Liang, Xiran and Xiong, Yingfei and Zhang, Lu},
  booktitle={Proceedings of the 35th IEEE/ACM International Conference on Automated Software Engineering},
  pages={883--894},
  year={2020}
}
@article{zheng2023survey,
  title={A survey of large language models for code: Evolution, benchmarking, and future trends},
  author={Zheng, Zibin and Ning, Kaiwen and Wang, Yanlin and Zhang, Jingwen and Zheng, Dewu and Ye, Mingxi and Chen, Jiachi},
  journal={arXiv preprint arXiv:2311.10372},
  year={2023}
}
@article{zheng2023towards,
  title={Towards an understanding of large language models in software engineering tasks},
  author={Zheng, Zibin and Ning, Kaiwen and Chen, Jiachi and Wang, Yanlin and Chen, Wenqing and Guo, Lianghong and Wang, Weicheng},
  journal={arXiv preprint arXiv:2308.11396},
  year={2023}
}
@inproceedings{du2021single,
  title={Is a single model enough? mucos: A multi-model ensemble learning approach for semantic code search},
  author={Du, Lun and Shi, Xiaozhou and Wang, Yanlin and Shi, Ensheng and Han, Shi and Zhang, Dongmei},
  booktitle={Proceedings of the 30th ACM International Conference on Information \& Knowledge Management},
  pages={2994--2998},
  year={2021}
}
@inproceedings{wan2019multi,
  title={Multi-modal attention network learning for semantic source code retrieval},
  author={Wan, Yao and Shu, Jingdong and Sui, Yulei and Xu, Guandong and Zhao, Zhou and Wu, Jian and Yu, Philip},
  booktitle={2019 34th IEEE/ACM International Conference on Automated Software Engineering (ASE)},
  pages={13--25},
  year={2019},
  organization={IEEE}
}
@article{ling2021deep,
  title={Deep graph matching and searching for semantic code retrieval},
  author={Ling, Xiang and Wu, Lingfei and Wang, Saizhuo and Pan, Gaoning and Ma, Tengfei and Xu, Fangli and Liu, Alex X and Wu, Chunming and Ji, Shouling},
  journal={ACM Transactions on Knowledge Discovery from Data (TKDD)},
  volume={15},
  number={5},
  pages={1--21},
  year={2021},
  publisher={ACM New York, NY, USA}
}

@inproceedings{ling2020adaptive,
  title={Adaptive deep code search},
  author={Ling, Chunyang and Lin, Zeqi and Zou, Yanzhen and Xie, Bing},
  booktitle={Proceedings of the 28th International Conference on Program Comprehension},
  pages={48--59},
  year={2020}
}
@article{cosqa,
  title={Cosqa: 20,000+ web queries for code search and question answering},
  author={Huang, Junjie and Tang, Duyu and Shou, Linjun and Gong, Ming and Xu, Ke and Jiang, Daxin and Zhou, Ming and Duan, Nan},
  journal={arXiv preprint arXiv:2105.13239},
  year={2021}
}
@inproceedings{yao2018staqc,
  title={Staqc: A systematically mined question-code dataset from stack overflow},
  author={Yao, Ziyu and Weld, Daniel S and Chen, Wei-Peng and Sun, Huan},
  booktitle={Proceedings of the 2018 World Wide Web Conference},
  pages={1693--1703},
  year={2018}
}
@online{wiki:MRR,
  author       = {Wikipedia contributors},
  title        = {MRR --- Wikipedia{,} The Free Encyclopedia},
  year         = {2024},
  url          = {https://en.wikipedia.org/wiki/MRR},
  note         = {[Online; accessed 2-August-2024]},
}

@article{csn,
  title={Codesearchnet challenge: Evaluating the state of semantic code search},
  author={Husain, Hamel and Wu, Ho-Hsiang and Gazit, Tiferet and Allamanis, Miltiadis and Brockschmidt, Marc},
  journal={arXiv preprint arXiv:1909.09436},
  year={2019}
}
@inproceedings{shi2023cocosoda,
  title={Cocosoda: Effective contrastive learning for code search},
  author={Shi, Ensheng and Wang, Yanlin and Gu, Wenchao and Du, Lun and Zhang, Hongyu and Han, Shi and Zhang, Dongmei and Sun, Hongbin},
  booktitle={2023 IEEE/ACM 45th International Conference on Software Engineering (ICSE)},
  pages={2198--2210},
  year={2023},
  organization={IEEE}
}
@article{codesurvey,
  title={Survey of code search based on deep learning},
  author={Xie, Yutao and Lin, Jiayi and Dong, Hande and Zhang, Lei and Wu, Zhonghai},
  journal={ACM Transactions on Software Engineering and Methodology},
  volume={33},
  number={2},
  pages={1--42},
  year={2023},
  publisher={ACM New York, NY}
}

@inproceedings{li2020learning,
  title={Learning code-query interaction for enhancing code searches},
  author={Li, Wei and Qin, Haozhe and Yan, Shuhan and Shen, Beijun and Chen, Yuting},
  booktitle={2020 IEEE International Conference on Software Maintenance and Evolution (ICSME)},
  pages={115--126},
  year={2020},
  organization={IEEE}
}
@misc{paperswithcode2024,
  author       = {{Papers with Code}},
  title        = {Code Generation on MBPP},
  year         = {2024},
  howpublished = {\url{https://paperswithcode.com/sota/code-generation-on-mbpp}},
  note         = {Accessed: August 1, 2024.}
}
@article{gong2024cosqa+,
  title={CoSQA+: Enhancing Code Search Dataset with Matching Code},
  author={Gong, Jing and Wu, Yanghui and Liang, Linxi and Zheng, Zibin and Wang, Yanlin},
  journal={arXiv preprint arXiv:2406.11589},
  year={2024}
}

@inproceedings{shuai2020improving,
  title={Improving code search with co-attentive representation learning},
  author={Shuai, Jianhang and Xu, Ling and Liu, Chao and Yan, Meng and Xia, Xin and Lei, Yan},
  booktitle={Proceedings of the 28th International Conference on Program Comprehension},
  pages={196--207},
  year={2020}
}
@inproceedings{ye2020leveraging,
  title={Leveraging code generation to improve code retrieval and summarization via dual learning},
  author={Ye, Wei and Xie, Rui and Zhang, Jinglei and Hu, Tianxiang and Wang, Xiaoyin and Zhang, Shikun},
  booktitle={Proceedings of The Web Conference 2020},
  pages={2309--2319},
  year={2020}
}



@inproceedings{gu2018deep,
  title={Deep code search},
  author={Gu, Xiaodong and Zhang, Hongyu and Kim, Sunghun},
  booktitle={Proceedings of the 40th International Conference on Software Engineering},
  pages={933--944},
  year={2018}
}


@inproceedings{ma2024fine,
  title={Fine-tuning llama for multi-stage text retrieval},
  author={Ma, Xueguang and Wang, Liang and Yang, Nan and Wei, Furu and Lin, Jimmy},
  booktitle={Proceedings of the 47th International ACM SIGIR Conference on Research and Development in Information Retrieval},
  pages={2421--2425},
  year={2024}
}


@article{E5wang2023improving,
  title={Improving text embeddings with large language models},
  author={Wang, Liang and Yang, Nan and Huang, Xiaolong and Yang, Linjun and Majumder, Rangan and Wei, Furu},
  journal={arXiv preprint arXiv:2401.00368},
  year={2023}
}



@article{gao2021simcse,
  title={Simcse: Simple contrastive learning of sentence embeddings},
  author={Gao, Tianyu and Yao, Xingcheng and Chen, Danqi},
  journal={arXiv preprint arXiv:2104.08821},
  year={2021}
}





@article{echoembeddingspringer2024repetition,
  title={Repetition improves language model embeddings},
  author={Springer, Jacob Mitchell and Kotha, Suhas and Fried, Daniel and Neubig, Graham and Raghunathan, Aditi},
  journal={arXiv preprint arXiv:2402.15449},
  year={2024}
}

@article{behnamghader2024llm2vec,
  title={Llm2vec: Large language models are secretly powerful text encoders},
  author={BehnamGhader, Parishad and Adlakha, Vaibhav and Mosbach, Marius and Bahdanau, Dzmitry and Chapados, Nicolas and Reddy, Siva},
  journal={arXiv preprint arXiv:2404.05961},
  year={2024}
}







@inproceedings{DBLP:conf/icse/YuLSR00L0W22,
  author    = {Hao Yu and
               Yiling Lou and
               Ke Sun and
               Dezhi Ran and
               Tao Xie and
               Dan Hao and
               Ying Li and
               Ge Li and
               Qianxiang Wang},
  title     = {Automated Assertion Generation via Information Retrieval and Its Integration
               with Deep learning},
  booktitle = {44th {IEEE/ACM} 44th International Conference on Software Engineering,
               {ICSE} 2022, Pittsburgh, PA, USA, May 25-27, 2022},
  pages     = {163--174},
  publisher = {{ACM}},
  year      = {2022},
  url       = {https://doi.org/10.1145/3510003.3510149},
  doi       = {10.1145/3510003.3510149}
}






@article{xie2023survey,
  title={Survey of code search based on deep learning},
  author={Xie, Yutao and Lin, Jiayi and Dong, Hande and Zhang, Lei and Wu, Zhonghai},
  journal={ACM Transactions on Software Engineering and Methodology},
  volume={33},
  number={2},
  pages={1--42},
  year={2023},
  publisher={ACM New York, NY}
}
















@inproceedings{DBLP:conf/icse/WatsonTMBP20,
  author    = {Cody Watson and
               Michele Tufano and
               Kevin Moran and
               Gabriele Bavota and
               Denys Poshyvanyk},
  editor    = {Gregg Rothermel and
               Doo{-}Hwan Bae},
  title     = {On learning meaningful assert statements for unit test cases},
  booktitle = {{ICSE} '20: 42nd International Conference on Software Engineering,
               Seoul, South Korea, 27 June - 19 July, 2020},
  pages     = {1398--1409},
  publisher = {{ACM}},
  year      = {2020},
  url       = {https://doi.org/10.1145/3377811.3380429},
  doi       = {10.1145/3377811.3380429}
}


@inproceedings{DBLP:conf/icse/DinellaRML22,
  author    = {Elizabeth Dinella and
               Gabriel Ryan and
               Todd Mytkowicz and
               Shuvendu K. Lahiri},
  title     = {{TOGA:} {A} Neural Method for Test Oracle Generation},
  booktitle = {44th {IEEE/ACM} 44th International Conference on Software Engineering,
               {ICSE} 2022, Pittsburgh, PA, USA, May 25-27, 2022},
  pages     = {2130--2141},
  publisher = {{ACM}},
  year      = {2022},
  url       = {https://doi.org/10.1145/3510003.3510141},
  doi       = {10.1145/3510003.3510141}
}


@inproceedings{DBLP:conf/icse/MastropaoloSCNP21,
  author    = {Antonio Mastropaolo and
               Simone Scalabrino and
               Nathan Cooper and
               David Nader{-}Palacio and
               Denys Poshyvanyk and
               Rocco Oliveto and
               Gabriele Bavota},
  title     = {Studying the Usage of Text-To-Text Transfer Transformer to Support
               Code-Related Tasks},
  booktitle = {43rd {IEEE/ACM} International Conference on Software Engineering,
               {ICSE} 2021, Madrid, Spain, 22-30 May 2021},
  pages     = {336--347},
  publisher = {{IEEE}},
  year      = {2021},
  url       = {https://doi.org/10.1109/ICSE43902.2021.00041},
  doi       = {10.1109/ICSE43902.2021.00041}
}

@article{DBLP:journals/tse/Mastropaolo22,
  author    = {Antonio Mastropaolo and
               Nathan Cooper and
               David Nader{-}Palacio and
               Simone Scalabrino and
               Denys Poshyvanyk and
               Rocco Oliveto and
               Gabriele Bavota},
  title     = {Using Transfer Learning for Code-Related Tasks},
  journal   = {IEEE Transactions on Software Engineering (TSE)},
  year      = {2022}
}

@inproceedings{DBLP:conf/ast/TufanoDSS22,
  author    = {Michele Tufano and
               Dawn Drain and
               Alexey Svyatkovskiy and
               Neel Sundaresan},
  title     = {Generating Accurate Assert Statements for Unit Test Cases using Pretrained
               Transformers},
  booktitle = {{IEEE/ACM} International Conference on Automation of Software Test,
               AST@ICSE 2022, Pittsburgh, PA, USA, May 21-22, 2022},
  pages     = {54--64},
  publisher = {{ACM/IEEE}},
  year      = {2022},
  url       = {https://doi.org/10.1145/3524481.3527220},
  doi       = {10.1145/3524481.3527220},
  timestamp = {Thu, 21 Jul 2022 13:37:46 +0200},
  biburl    = {https://dblp.org/rec/conf/ast/TufanoDSS22.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@inproceedings{DBLP:conf/nips/VaswaniSPUJGKP17,
  author    = {Ashish Vaswani and
               Noam Shazeer and
               Niki Parmar and
               Jakob Uszkoreit and
               Llion Jones and
               Aidan N. Gomez and
               Lukasz Kaiser and
               Illia Polosukhin},
  editor    = {Isabelle Guyon and
               Ulrike von Luxburg and
               Samy Bengio and
               Hanna M. Wallach and
               Rob Fergus and
               S. V. N. Vishwanathan and
               Roman Garnett},
  title     = {Attention is All you Need},
  booktitle = {Advances in Neural Information Processing Systems 30: Annual Conference
               on Neural Information Processing Systems 2017, December 4-9, 2017,
               Long Beach, CA, {USA}},
  pages     = {5998--6008},
  year      = {2017},
}

@inproceedings{DBLP:conf/emnlp/0034WJH21,
  author    = {Yue Wang and
               Weishi Wang and
               Shafiq R. Joty and
               Steven C. H. Hoi},
  editor    = {Marie{-}Francine Moens and
               Xuanjing Huang and
               Lucia Specia and
               Scott Wen{-}tau Yih},
  title     = {CodeT5: Identifier-aware Unified Pre-trained Encoder-Decoder Models
               for Code Understanding and Generation},
  booktitle = {Proceedings of the 2021 Conference on Empirical Methods in Natural
               Language Processing, {EMNLP} 2021, Virtual Event / Punta Cana, Dominican
               Republic, 7-11 November, 2021},
  pages     = {8696--8708},
  publisher = {Association for Computational Linguistics},
  year      = {2021},
  url       = {https://doi.org/10.18653/v1/2021.emnlp-main.685},
  doi       = {10.18653/v1/2021.emnlp-main.685}
}

@article{taylor1953cloze,
  title={“Cloze procedure”: A new tool for measuring readability},
  author={Taylor, Wilson L},
  journal={Journalism quarterly},
  volume={30},
  number={4},
  pages={415--433},
  year={1953},
  publisher={SAGE Publications Sage CA: Los Angeles, CA}
}


@inproceedings{DBLP:conf/naacl/DevlinCLT19,
  author    = {Jacob Devlin and
               Ming{-}Wei Chang and
               Kenton Lee and
               Kristina Toutanova},
  editor    = {Jill Burstein and
               Christy Doran and
               Thamar Solorio},
  title     = {{BERT:} Pre-training of Deep Bidirectional Transformers for Language
               Understanding},
  booktitle = {Proceedings of the 2019 Conference of the North American Chapter of
               the Association for Computational Linguistics: Human Language Technologies,
               {NAACL-HLT} 2019, Minneapolis, MN, USA, June 2-7, 2019, Volume 1 (Long
               and Short Papers)},
  pages     = {4171--4186},
  publisher = {Association for Computational Linguistics},
  year      = {2019},
  url       = {https://doi.org/10.18653/v1/n19-1423},
  doi       = {10.18653/v1/n19-1423}
}


@inproceedings{DBLP:conf/emnlp/FengGTDFGS0LJZ20,
  author    = {Zhangyin Feng and
               Daya Guo and
               Duyu Tang and
               Nan Duan and
               Xiaocheng Feng and
               Ming Gong and
               Linjun Shou and
               Bing Qin and
               Ting Liu and
               Daxin Jiang and
               Ming Zhou},
  editor    = {Trevor Cohn and
               Yulan He and
               Yang Liu},
  title     = {CodeBERT: {A} Pre-Trained Model for Programming and Natural Languages},
  booktitle = {Findings of the Association for Computational Linguistics: {EMNLP}
               2020, Online Event, 16-20 November 2020},
  series    = {Findings of {ACL}},
  volume    = {{EMNLP} 2020},
  pages     = {1536--1547},
  publisher = {Association for Computational Linguistics},
  year      = {2020},
  url       = {https://doi.org/10.18653/v1/2020.findings-emnlp.139},
  doi       = {10.18653/v1/2020.findings-emnlp.139}
}


@article{DBLP:journals/corr/abs-2203-13474,
  author    = {Erik Nijkamp and
               Bo Pang and
               Hiroaki Hayashi and
               Lifu Tu and
               Huan Wang and
               Yingbo Zhou and
               Silvio Savarese and
               Caiming Xiong},
  title     = {A Conversational Paradigm for Program Synthesis},
  journal   = {CoRR},
  volume    = {abs/2203.13474},
  year      = {2022},
  url       = {https://doi.org/10.48550/arXiv.2203.13474},
  doi       = {10.48550/arXiv.2203.13474}
}

@inproceedings{DBLP:conf/kbse/TanejaX08,
  author    = {Kunal Taneja and
               Tao Xie},
  title     = {DiffGen: Automated Regression Unit-Test Generation},
  booktitle = {23rd {IEEE/ACM} International Conference on Automated Software Engineering
               {(ASE} 2008), 15-19 September 2008, L'Aquila, Italy},
  pages     = {407--410},
  publisher = {{IEEE} Computer Society},
  year      = {2008},
  url       = {https://doi.org/10.1109/ASE.2008.60},
  doi       = {10.1109/ASE.2008.60}
}

@inproceedings{DBLP:conf/sigsoft/FraserA11,
  author    = {Gordon Fraser and
               Andrea Arcuri},
  editor    = {Tibor Gyim{\'{o}}thy and
               Andreas Zeller},
  title     = {EvoSuite: automatic test suite generation for object-oriented software},
  booktitle = {SIGSOFT/FSE'11 19th {ACM} {SIGSOFT} Symposium on the Foundations of
               Software Engineering {(FSE-19)} and ESEC'11: 13th European Software
               Engineering Conference (ESEC-13), Szeged, Hungary, September 5-9,
               2011},
  pages     = {416--419},
  publisher = {{ACM}},
  year      = {2011},
  url       = {https://doi.org/10.1145/2025113.2025179},
  doi       = {10.1145/2025113.2025179}
}

@inproceedings{DBLP:conf/oopsla/PachecoE07,
  author    = {Carlos Pacheco and
               Michael D. Ernst},
  editor    = {Richard P. Gabriel and
               David F. Bacon and
               Cristina Videira Lopes and
               Guy L. Steele Jr.},
  title     = {Randoop: feedback-directed random testing for Java},
  booktitle = {Companion to the 22nd Annual {ACM} {SIGPLAN} Conference on Object-Oriented
               Programming, Systems, Languages, and Applications, {OOPSLA} 2007,
               October 21-25, 2007, Montreal, Quebec, Canada},
  pages     = {815--816},
  publisher = {{ACM}},
  year      = {2007},
  url       = {https://doi.org/10.1145/1297846.1297902},
  doi       = {10.1145/1297846.1297902}
}

@inproceedings{DBLP:conf/icse/AlmasiHFAB17,
  author    = {Mohammad Moein Almasi and
               Hadi Hemmati and
               Gordon Fraser and
               Andrea Arcuri and
               Janis Benefelds},
  title     = {An Industrial Evaluation of Unit Test Generation: Finding Real Faults
               in a Financial Application},
  booktitle = {39th {IEEE/ACM} International Conference on Software Engineering:
               Software Engineering in Practice Track, {ICSE-SEIP} 2017, Buenos Aires,
               Argentina, May 20-28, 2017},
  pages     = {263--272},
  publisher = {{IEEE} Computer Society},
  year      = {2017},
  url       = {https://doi.org/10.1109/ICSE-SEIP.2017.27},
  doi       = {10.1109/ICSE-SEIP.2017.27}
}



@inproceedings{DBLP:conf/sigsoft/Shamshiri15,
  author    = {Sina Shamshiri},
  editor    = {Elisabetta Di Nitto and
               Mark Harman and
               Patrick Heymans},
  title     = {Automated unit test generation for evolving software},
  booktitle = {Proceedings of the 2015 10th Joint Meeting on Foundations of Software
               Engineering, {ESEC/FSE} 2015, Bergamo, Italy, August 30 - September
               4, 2015},
  pages     = {1038--1041},
  publisher = {{ACM}},
  year      = {2015},
  url       = {https://doi.org/10.1145/2786805.2803196},
  doi       = {10.1145/2786805.2803196}
}


@inproceedings{DBLP:conf/nips/ConneauL19,
  author    = {Alexis Conneau and
               Guillaume Lample},
  editor    = {Hanna M. Wallach and
               Hugo Larochelle and
               Alina Beygelzimer and
               Florence d'Alch{\'{e}}{-}Buc and
               Emily B. Fox and
               Roman Garnett},
  title     = {Cross-lingual Language Model Pretraining},
  booktitle = {Advances in Neural Information Processing Systems 32: Annual Conference
               on Neural Information Processing Systems 2019, NeurIPS 2019, December
               8-14, 2019, Vancouver, BC, Canada},
  pages     = {7057--7067},
  year      = {2019}
}


@misc{junitpopular,
    author = "{Yolande Poirier}",
    title = {{What are the Most Popular Libraries Java Developers Use? Based on Github’s Top Projects.}},
    howpublished = {\url{https://blogs.oracle.com/java/top-java-libraries-on-github}},
}

@article{arXiv21chatgptfixbug,
  title={An analysis of the automatic bug fixing performance of chatgpt},
  author={Sobania, Dominik and Briesch, Martin and Hanna, Carol and Petke, Justyna},
  journal={arXiv preprint arXiv:2301.08653},
  year={2023}
}

@article{arXiv23chatgptrepair,
  title={A study on Prompt Design, Advantages and Limitations of ChatGPT for Deep Learning Program Repair},
  author={Cao, Jialun and Li, Meiziniu and Wen, Ming and Cheung, Shing-chi},
  journal={arXiv preprint arXiv:2304.08191},
  year={2023}
}

@article{kang2023explainable,
  title={Explainable Automated Debugging via Large Language Model-driven Scientific Debugging},
  author={Kang, Sungmin and Chen, Bei and Yoo, Shin and Lou, Jian-Guang},
  journal={arXiv preprint arXiv:2304.02195},
  year={2023}
}

% related work

@misc{arXiv23ChatgptProgrammingAssistant,
      title={Is ChatGPT the Ultimate Programming Assistant -- How far is it?}, 
      author={Haoye Tian and Weiqi Lu and Tsz On Li and Xunzhu Tang and Shing-Chi Cheung and Jacques Klein and Tegawendé F. Bissyandé},
      year={2023},
      eprint={2304.11938},
      archivePrefix={arXiv},
      primaryClass={cs.SE}
}

@article{arXiv23ConversationalProgramRepair,
  title={Conversational automated program repair},
  author={Xia, Chunqiu Steven and Zhang, Lingming},
  journal={arXiv preprint arXiv:2301.13246},
  year={2023}
}

@misc{arXiv23AutomaticBugFixing,
      title={An Analysis of the Automatic Bug Fixing Performance of ChatGPT}, 
      author={Dominik Sobania and Martin Briesch and Carol Hanna and Justyna Petke},
      year={2023},
      eprint={2301.08653},
      archivePrefix={arXiv},
      primaryClass={cs.SE}
}

@misc{prenner2021automatic,
      title={Automatic Program Repair with OpenAI's Codex: Evaluating QuixBugs}, 
      author={Julian Aron Prenner and Romain Robbes},
      year={2021},
      eprint={2111.03922},
      archivePrefix={arXiv},
      primaryClass={cs.SE}
}

@inproceedings{wang2023automatically,
  title={Automatically Resolving Dependency-Conflict Building Failures via Behavior-Consistent Loosening of Library Version Constraints},
  author={Wang, Huiyan and Liu, Shuguan and Zhang, Lingyu and Xu, Chang},
  booktitle={Proceedings of the 31st ACM Joint European Software Engineering Conference and Symposium on the Foundations of Software Engineering},
  pages={198--210},
  year={2023}
}

@inproceedings{Zhao23Knowledge,
author = {Zhao, Zhongkai and Kou, Bonan and Ibrahim, Mohamed Yilmaz and Chen, Muhao and Zhang, Tianyi},
title = {Knowledge-Based Version Incompatibility Detection for Deep Learning},
year = {2023},
isbn = {9798400703270},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3611643.3616364},
doi = {10.1145/3611643.3616364},
booktitle = {Proceedings of the 31st ACM Joint European Software Engineering Conference and Symposium on the Foundations of Software Engineering},
pages = {708–719},
numpages = {12},
keywords = {Version Compatibility, Knowledge Extraction, Deep Learning},
location = {, San Francisco, CA, USA, },
series = {ESEC/FSE 2023}
}



@inproceedings{QuixBug,
author = {Lin, Derrick and Koppel, James and Chen, Angela and Solar-Lezama, Armando},
title = {QuixBugs: A Multi-Lingual Program Repair Benchmark Set Based on the Quixey Challenge},
year = {2017},
isbn = {9781450355148},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3135932.3135941},
doi = {10.1145/3135932.3135941},
abstract = {Recent years have seen an explosion of work in automated program repair. While previous work has focused exclusively on tools for single languages, recent work in multi-language transformation has opened the door for multi-language program repair tools. Evaluating the performance of such a tool requires having a benchmark set of similar buggy programs in different languages. We present QuixBugs, consisting of 40 programs translated to both Python and Java, each with a bug on a single line. The QuixBugs benchmark suite is based on problems from the Quixey Challenge, where programmers were given a short buggy program and 1 minute to fix the bug.},
booktitle = {Proceedings Companion of the 2017 ACM SIGPLAN International Conference on Systems, Programming, Languages, and Applications: Software for Humanity},
pages = {55–56},
numpages = {2},
keywords = {automated program repair, benchmark},
location = {Vancouver, BC, Canada},
series = {SPLASH Companion 2017}
}


@misc{mavencenter,
	title = {{Maven} {Central} {Repository}},
	url = {https://mvnrepository.com},
	year = {2022},
	lastaccessed = {January 20, 2023}
}


@misc{prompts,
	title = {chatgpt-prompts},
	url = {https://github.com/f/awesome-chatgpt-prompts},
	year = {2023}
}

@misc{chatgpt,
	title = {chatgpt},
	url = {https://chat.openai.com/},
	year = {2022},
        publisher = {{OpenAI}}
}

@article{openai2023gpt4,
  author       = {OpenAI},
  title        = {{GPT-4} Technical Report},
  journal      = {CoRR},
  volume       = {abs/2303.08774},
  year         = {2023},
  url          = {https://doi.org/10.48550/arXiv.2303.08774},
  doi          = {10.48550/arXiv.2303.08774},
  eprinttype    = {arXiv},
  eprint       = {2303.08774},
  timestamp    = {Mon, 20 Mar 2023 15:23:19 +0100},
  biburl       = {https://dblp.org/rec/journals/corr/abs-2303-08774.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@misc{claude,
	title = {Claude},
	url = {https://www.anthropic.com/index/introducing-claude},
	year = {2023},
        publisher = {{Anthropic}}
}

@misc{bard,
	title = {Bard},
	url = {https://bard.google.com/},
	year = {2023},
        publisher = {{Google}}
}

@article{luo2023wizardcoder,
  author       = {Ziyang Luo and
                  Can Xu and
                  Pu Zhao and
                  Qingfeng Sun and
                  Xiubo Geng and
                  Wenxiang Hu and
                  Chongyang Tao and
                  Jing Ma and
                  Qingwei Lin and
                  Daxin Jiang},
  title        = {WizardCoder: Empowering Code Large Language Models with Evol-Instruct},
  journal      = {CoRR},
  volume       = {abs/2306.08568},
  year         = {2023},
  url          = {https://doi.org/10.48550/arXiv.2306.08568},
  doi          = {10.48550/arXiv.2306.08568},
  eprinttype    = {arXiv},
  eprint       = {2306.08568},
  timestamp    = {Sun, 18 Jun 2023 16:10:59 +0200},
  biburl       = {https://dblp.org/rec/journals/corr/abs-2306-08568.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{codellama,
  title={Code llama: Open foundation models for code},
  author={Rozi{\`e}re, Baptiste and Gehring, Jonas and Gloeckle, Fabian and Sootla, Sten and Gat, Itai and Tan, Xiaoqing Ellen and Adi, Yossi and Liu, Jingyu and Remez, Tal and Rapin, J{\'e}r{\'e}my and others},
  journal={arXiv preprint arXiv:2308.12950},
  year={2023}
}

@misc{du2023classeval,
      title={ClassEval: A Manually-Crafted Benchmark for Evaluating LLMs on Class-level Code Generation}, 
      author={Xueying Du and Mingwei Liu and Kaixin Wang and Hanlin Wang and Junwei Liu and Yixuan Chen and Jiayi Feng and Chaofeng Sha and Xin Peng and Yiling Lou},
      year={2023},
      eprint={2308.01861},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}

@article{humaneval,
  author       = {Mark Chen and
                  Jerry Tworek and
                  Heewoo Jun and
                  Qiming Yuan and
                  Henrique Pond{\'{e}} de Oliveira Pinto and
                  Jared Kaplan and
                  Harrison Edwards and
                  Yuri Burda and
                  Nicholas Joseph and
                  Greg Brockman and
                  Alex Ray and
                  Raul Puri and
                  Gretchen Krueger and
                  Michael Petrov and
                  Heidy Khlaaf and
                  Girish Sastry and
                  Pamela Mishkin and
                  Brooke Chan and
                  Scott Gray and
                  Nick Ryder and
                  Mikhail Pavlov and
                  Alethea Power and
                  Lukasz Kaiser and
                  Mohammad Bavarian and
                  Clemens Winter and
                  Philippe Tillet and
                  Felipe Petroski Such and
                  Dave Cummings and
                  Matthias Plappert and
                  Fotios Chantzis and
                  Elizabeth Barnes and
                  Ariel Herbert{-}Voss and
                  William Hebgen Guss and
                  Alex Nichol and
                  Alex Paino and
                  Nikolas Tezak and
                  Jie Tang and
                  Igor Babuschkin and
                  Suchir Balaji and
                  Shantanu Jain and
                  William Saunders and
                  Christopher Hesse and
                  Andrew N. Carr and
                  Jan Leike and
                  Joshua Achiam and
                  Vedant Misra and
                  Evan Morikawa and
                  Alec Radford and
                  Matthew Knight and
                  Miles Brundage and
                  Mira Murati and
                  Katie Mayer and
                  Peter Welinder and
                  Bob McGrew and
                  Dario Amodei and
                  Sam McCandlish and
                  Ilya Sutskever and
                  Wojciech Zaremba},
  title        = {Evaluating Large Language Models Trained on Code},
  journal      = {CoRR},
  volume       = {abs/2107.03374},
  year         = {2021},
  url          = {https://arxiv.org/abs/2107.03374},
  eprinttype    = {arXiv},
  eprint       = {2107.03374},
  timestamp    = {Thu, 25 May 2023 10:38:31 +0200},
  biburl       = {https://dblp.org/rec/journals/corr/abs-2107-03374.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}


@misc{replication_package,
	title = {replication package},
	url = {https://llm4crasolver.github.io},
	year = {2024}
}

@misc{68199510,
	title = {the Stack Overflow post ID of the crash bug},
	url = {https://stackoverflow.com/questions/68199510},
	year = {2023}
}

@misc{65084069,
	title = {the Stack Overflow post ID of the crash bug},
	url = {https://stackoverflow.com/questions/65084069},
	year = {2023}
}

@misc{22928450,
	title = {the Stack Overflow post ID of the crash bug},
	url = {https://stackoverflow.com/questions/22928450},
	year = {2023}
}

@misc{28097042,
	title = {the Stack Overflow post ID of the crash bug},
	url = {https://stackoverflow.com/questions/28097042},
	year = {2023}
}

@misc{24305296,
	title = {the Stack Overflow post ID of the crash bug},
	url = {https://stackoverflow.com/questions/24305296},
	year = {2023}
}

@misc{49871007,
	title = {the Stack Overflow post ID of the crash bug},
	url = {https://stackoverflow.com/questions/49871007},
	year = {2023}
}

@misc{37771758,
	title = {the Stack Overflow post ID of the crash bug},
	url = {https://stackoverflow.com/questions/37771758},
	year = {2023}
}

@misc{43320334,
	title = {the Stack Overflow post ID of the crash bug},
	url = {https://stackoverflow.com/questions/43320334},
	year = {2023}
}




@misc{so_dump,
	url = {https://archive.org/download/stackexchange/},
	title = {Stack Overflow data dump version from September 4, 2021},
	year = {2021},
	lastaccessed = {May 4, 2022}
} 
@inproceedings{icse21crasolver,
  author    = {Haoye Wang and
               Xin Xia and
               David Lo and
               John C. Grundy and
               Xinyu Wang},
  title     = {Automatic Solution Summarization for Crash Bugs},
  booktitle = {43rd {IEEE/ACM} International Conference on Software Engineering,
               {ICSE} 2021, Madrid, Spain, 22-30 May 2021},
  pages     = {1286--1297},
  publisher = {{IEEE}},
  year      = {2021}
}
@inproceedings{fse20masetro,
  author    = {Sonal Mahajan and
               Negarsadat Abolhassani and
               Mukul R. Prasad},
  title     = {Recommending stack overflow posts for fixing runtime exceptions using
               failure scenario matching},
  booktitle = {{ESEC/FSE} '20: 28th {ACM} Joint European Software Engineering Conference
               and Symposium on the Foundations of Software Engineering, Virtual
               Event, USA, November 8-13, 2020},
  pages     = {1052--1064},
  publisher = {{ACM}},
  year      = {2020}
}
@misc{libariesiodata,
	title = {Libaries.io open data},
	url = {https://libraries.io/data},
	year = {2022},
	lastaccessed = {January 20, 2023}
}
@misc{java_api,
	url = {https://docs.oracle.com/javase/8/docs/api/overview-summary.html/},
    title={JDK 1.8},
    year = {2023}
} 
@article{kappa,
	title={Interrater reliability: the kappa statistic},
	author={McHugh, Mary L},
	journal={Biochemia Medica: Biochemia Medica},
	volume={22},
	number={3},
	pages={276--282},
	year={2012},
	publisher={Medicinska naklada}
}

@article{Likert1932,
	author = {Likert, Rensis},
	title = {{A technique for the measurement of attitudes.}},
	journal = {Archives of psychology},
	year = {1932}
}

@article{dong2023self,
  title={Self-collaboration Code Generation via ChatGPT},
  author={Dong, Yihong and Jiang, Xue and Jin, Zhi and Li, Ge},
  journal={arXiv preprint arXiv:2304.07590},
  year={2023}
}

@misc{poesia2022codegeneration,
      title={Synchromesh: Reliable code generation from pre-trained language models}, 
      author={Gabriel Poesia and Oleksandr Polozov and Vu Le and Ashish Tiwari and Gustavo Soares and Christopher Meek and Sumit Gulwani},
      year={2022},
      eprint={2201.11227},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}

@inproceedings{zeng2022codegeneration,
  title={An extensive study on pre-trained models for program understanding and generation},
  author={Zeng, Zhengran and Tan, Hanzhuo and Zhang, Haotian and Li, Jing and Zhang, Yuqun and Zhang, Lingming},
  booktitle={Proceedings of the 31st ACM SIGSOFT International Symposium on Software Testing and Analysis},
  pages={39--51},
  year={2022}
}

@inproceedings{hu2019apr,
  title={Re-factoring based program repair applied to programming assignments},
  author={Hu, Yang and Ahmed, Umair Z and Mechtaev, Sergey and Leong, Ben and Roychoudhury, Abhik},
  booktitle={2019 34th IEEE/ACM International Conference on Automated Software Engineering (ASE)},
  pages={388--398},
  year={2019},
  organization={IEEE}
}

@article{icse2023apr,
  author       = {Nan Jiang and
                  Kevin Liu and
                  Thibaud Lutellier and
                  Lin Tan},
  title        = {Impact of Code Language Models on Automated Program Repair},
  journal      = {CoRR},
  volume       = {abs/2302.05020},
  year         = {2023},
  url          = {https://doi.org/10.48550/arXiv.2302.05020},
  doi          = {10.48550/arXiv.2302.05020},
  eprinttype    = {arXiv},
  eprint       = {2302.05020},
  timestamp    = {Tue, 21 Mar 2023 21:05:23 +0100},
  biburl       = {https://dblp.org/rec/journals/corr/abs-2302-05020.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@INPROCEEDINGS{msr21apr,
  author={Mashhadi, Ehsan and Hemmati, Hadi},
  booktitle={2021 IEEE/ACM 18th International Conference on Mining Software Repositories (MSR)}, 
  title={Applying CodeBERT for Automated Program Repair of Java Simple Bugs}, 
  year={2021},
  volume={},
  number={},
  pages={505-509},
  doi={10.1109/MSR52588.2021.00063}}

@inproceedings{23codesummarization,
author = {Ahmed, Toufique and Devanbu, Premkumar},
title = {Few-Shot Training LLMs for Project-Specific Code-Summarization},
year = {2023},
isbn = {9781450394758},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3551349.3559555},
doi = {10.1145/3551349.3559555},
booktitle = {Proceedings of the 37th IEEE/ACM International Conference on Automated Software Engineering},
articleno = {177},
numpages = {5},
keywords = {deep learning, code summarization, large language model},
location = {Rochester, MI, USA},
series = {ASE '22}
}

@article{wang2020codesummarization,
  title={Fret: Functional reinforced transformer with bert for code summarization},
  author={Wang, Ruyun and Zhang, Hanwen and Lu, Guoliang and Lyu, Lei and Lyu, Chen},
  journal={IEEE Access},
  volume={8},
  pages={135591--135604},
  year={2020},
  publisher={IEEE}
}

@misc{davis2023mathematics,
      title={Mathematics, word problems, common sense, and artificial intelligence}, 
      author={Ernest Davis},
      year={2023},
      eprint={2301.09723},
      archivePrefix={arXiv},
      primaryClass={cs.AI}
}

@misc{frieder2023mathematical,
      title={Mathematical Capabilities of ChatGPT}, 
      author={Simon Frieder and Luca Pinchetti and Ryan-Rhys Griffiths and Tommaso Salvatori and Thomas Lukasiewicz and Philipp Christian Petersen and Alexis Chevalier and Julius Berner},
      year={2023},
      eprint={2301.13867},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}


@misc{bang2023nlp,
      title={A Multitask, Multilingual, Multimodal Evaluation of ChatGPT on Reasoning, Hallucination, and Interactivity}, 
      author={Yejin Bang and Samuel Cahyawijaya and Nayeon Lee and Wenliang Dai and Dan Su and Bryan Wilie and Holy Lovenia and Ziwei Ji and Tiezheng Yu and Willy Chung and Quyet V. Do and Yan Xu and Pascale Fung},
      year={2023},
      eprint={2302.04023},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}

@article{gilson2022education,
  title={How Well Does ChatGPT Do When Taking the Medical Licensing Exams? The Implications of Large Language Models for Medical Education and Knowledge Assessment},
  author={Gilson, Aidan and Safranek, Conrad and Huang, Thomas and Socrates, Vimig and Chi, Ling and Taylor, Richard Andrew and Chartash, David},
  journal={medRxiv},
  pages={2022--12},
  year={2022},
  publisher={Cold Spring Harbor Laboratory Press}
}

@article{baidoo2023education,
  title={Education in the era of generative artificial intelligence (AI): Understanding the potential benefits of ChatGPT in promoting teaching and learning},
  author={Baidoo-Anu, David and Owusu Ansah, Leticia},
  journal={Available at SSRN 4337484},
  year={2023}
}

@article{jiao2023nlp,
  title={Is ChatGPT a good translator? A preliminary study},
  author={Jiao, Wenxiang and Wang, Wenxuan and Huang, Jen-tse and Wang, Xing and Tu, Zhaopeng},
  journal={arXiv preprint arXiv:2301.08745},
  year={2023}
}

@article{jin2023inferfix,
  title={Inferfix: End-to-end program repair with llms},
  author={Jin, Matthew and Shahriar, Syed and Tufano, Michele and Shi, Xin and Lu, Shuai and Sundaresan, Neel and Svyatkovskiy, Alexey},
  journal={arXiv preprint arXiv:2303.07263},
  year={2023}
}


@inproceedings{icst22masetroextend,
  author    = {Sonal Mahajan and
               Mukul R. Prasad},
  title     = {Providing Real-time Assistance for Repairing Runtime Exceptions using
               Stack Overflow Posts},
  booktitle = {15th {IEEE} Conference on Software Testing, Verification and Validation,
               {ICST} 2022, Valencia, Spain, April 4-14, 2022},
  pages     = {196--207},
  publisher = {{IEEE}},
  year      = {2022}
}

@inproceedings{ferenc2018public,
  title={A public unified bug dataset for java},
  author={Ferenc, Rudolf and T{\'o}th, Zolt{\'a}n and Lad{\'a}nyi, Gergely and Siket, Istv{\'a}n and Gyim{\'o}thy, Tibor},
  booktitle={Proceedings of the 14th international conference on predictive models and data analytics in software engineering},
  pages={12--21},
  year={2018}
}

@inproceedings{karampatsis2020often,
  title={How often do single-statement bugs occur? the manysstubs4j dataset},
  author={Karampatsis, Rafael-Michael and Sutton, Charles},
  booktitle={Proceedings of the 17th International Conference on Mining Software Repositories},
  pages={573--577},
  year={2020}
}

@inproceedings{issta2014Defects4J,
   author = {Ren{\'e} Just and Darioush Jalali and Michael D. Ernst},
   title = {{Defects4J}: A {Database} of existing faults to enable
	controlled testing studies for {Java} programs},
   booktitle = {ISSTA 2014, Proceedings of the 2014 International
	Symposium on Software Testing and Analysis},
   pages = {437--440},
   address = {San Jose, CA, USA},
   month = jul,
   year = {2014},
   note = {Tool demo}
}

@article{white2023prompt,
  title={A prompt pattern catalog to enhance prompt engineering with chatgpt},
  author={White, Jules and Fu, Quchen and Hays, Sam and Sandborn, Michael and Olea, Carlos and Gilbert, Henry and Elnashar, Ashraf and Spencer-Smith, Jesse and Schmidt, Douglas C},
  journal={arXiv preprint arXiv:2302.11382},
  year={2023}
}

@inproceedings{icse22fl,
author = {Ciborowska, Agnieszka and Damevski, Kostadin},
title = {Fast Changeset-Based Bug Localization with BERT},
year = {2022},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
doi = {10.1145/3510003.3510042},
booktitle = {Proceedings of the 44th International Conference on Software Engineering},
pages = {946–957},
numpages = {12},
location = {Pittsburgh, Pennsylvania},
series = {ICSE '22}
}

@inproceedings{ase2021fl,
  title={Incbl: Incremental bug localization},
  author={Yang, Zhou and Shi, Jieke and Wang, Shaowei and Lo, David},
  booktitle={2021 36th IEEE/ACM International Conference on Automated Software Engineering (ASE)},
  pages={1223--1226},
  year={2021},
  organization={IEEE}
}

@inproceedings{cao2020fl,
  title={Bugpecker: Locating faulty methods with deep learning on revision graphs},
  author={Cao, Junming and Yang, Shouliang and Jiang, Wenhui and Zeng, Hushuang and Shen, Beijun and Zhong, Hao},
  booktitle={Proceedings of the 35th IEEE/ACM International Conference on Automated Software Engineering},
  pages={1214--1218},
  year={2020}
}

@article{Lin2017QuixBugsAM,
  title={QuixBugs: a multi-lingual program repair benchmark set based on the quixey challenge},
  author={Derrick Lin and James Koppel and Angela Chen and Armando Solar-Lezama},
  journal={Proceedings Companion of the 2017 ACM SIGPLAN International Conference on Systems, Programming, Languages, and Applications: Software for Humanity},
  year={2017},
  url={https://api.semanticscholar.org/CorpusID:7158771}
}

@inproceedings{ase15crashresolve,
  author    = {Qing Gao and
               Hansheng Zhang and
               Jie Wang and
               Yingfei Xiong and
               Lu Zhang and
               Hong Mei},
  editor    = {Myra B. Cohen and
               Lars Grunske and
               Michael Whalen},
  title     = {Fixing Recurring Crash Bugs via Analyzing Q{\&}A Sites {(T)}},
  booktitle = {30th {IEEE/ACM} International Conference on Automated Software Engineering,
               {ASE} 2015, Lincoln, NE, USA, November 9-13, 2015},
  pages     = {307--318},
  publisher    = {{IEEE} Computer Society},
  year         = {2015},
  url          = {https://doi.org/10.1109/ASE.2015.81},
  doi          = {10.1109/ASE.2015.81},
  timestamp    = {Tue, 09 May 2023 08:00:06 +0200},
  biburl       = {https://dblp.org/rec/conf/kbse/GaoZWXZM15.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}


@inproceedings{icsm11crashresolve2,
  author    = {Tejinder Dhaliwal and
               Foutse Khomh and
               Ying Zou},
  title     = {Classifying field crash reports for fixing bugs: {A} case study of
               Mozilla Firefox},
  booktitle = {{IEEE} 27th International Conference on Software Maintenance, {ICSM}
               2011, Williamsburg, VA, USA, September 25-30, 2011},
  pages     = {333--342},
  publisher    = {{IEEE} Computer Society},
  year         = {2011},
  url          = {https://doi.org/10.1109/ICSM.2011.6080800},
  doi          = {10.1109/ICSM.2011.6080800},
  timestamp    = {Fri, 24 Mar 2023 00:04:11 +0100},
  biburl       = {https://dblp.org/rec/conf/icsm/DhaliwalKZ11.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}


@article{yuan2023evaluating,
  title={Evaluating instruction-tuned large language models on code comprehension and generation},
  author={Yuan, Zhiqiang and Liu, Junwei and Zi, Qiancheng and Liu, Mingwei and Peng, Xin and Lou, Yiling},
  journal={arXiv preprint arXiv:2308.01240},
  year={2023}
}

@article{hou2023large,
  title={Large language models for software engineering: A systematic literature review},
  author={Hou, Xinyi and Zhao, Yanjie and Liu, Yue and Yang, Zhou and Wang, Kailong and Li, Li and Luo, Xiapu and Lo, David and Grundy, John and Wang, Haoyu},
  journal={arXiv preprint arXiv:2308.10620},
  year={2023}
}


@misc{min2022rethinking,
      title={Rethinking the Role of Demonstrations: What Makes In-Context Learning Work?}, 
      author={Sewon Min and Xinxi Lyu and Ari Holtzman and Mikel Artetxe and Mike Lewis and Hannaneh Hajishirzi and Luke Zettlemoyer},
      year={2022},
      eprint={2202.12837},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}

@article{wei2023chainofthought,
  title={Chain-of-thought prompting elicits reasoning in large language models},
  author={Wei, Jason and Wang, Xuezhi and Schuurmans, Dale and Bosma, Maarten and Xia, Fei and Chi, Ed and Le, Quoc V and Zhou, Denny and others},
  journal={Advances in Neural Information Processing Systems},
  volume={35},
  pages={24824--24837},
  year={2022}
}

@article{zhang2022automatic,
  title={Automatic chain of thought prompting in large language models},
  author={Zhang, Zhuosheng and Zhang, Aston and Li, Mu and Smola, Alex},
  journal={arXiv preprint arXiv:2210.03493},
  year={2022}
}

@article{liu2022generated,
  title={Generated knowledge prompting for commonsense reasoning},
  author={Liu, Jiacheng and Liu, Alisa and Lu, Ximing and Welleck, Sean and West, Peter and Bras, Ronan Le and Choi, Yejin and Hajishirzi, Hannaneh},
  journal={arXiv preprint arXiv:2110.08387},
  year={2022}
}


@article{yao2023tree,
  title={Tree of thoughts: Deliberate problem solving with large language models},
  author={Yao, Shunyu and Yu, Dian and Zhao, Jeffrey and Shafran, Izhak and Griffiths, Thomas L and Cao, Yuan and Narasimhan, Karthik},
  journal={arXiv preprint arXiv:2305.10601},
  year={2023}
}

@article{liu2023improving,
  title={Improving ChatGPT Prompt for Code Generation},
  author={Liu, Chao and Bao, Xuanlin and Zhang, Hongyu and Zhang, Neng and Hu, Haibo and Zhang, Xiaohong and Yan, Meng},
  journal={arXiv preprint arXiv:2305.08360},
  year={2023}
}

@misc{yuan2023manual,
      title={No More Manual Tests? Evaluating and Improving ChatGPT for Unit Test Generation}, 
      author={Zhiqiang Yuan and Yiling Lou and Mingwei Liu and Shiji Ding and Kaixin Wang and Yixuan Chen and Xin Peng},
      year={2023},
      eprint={2305.04207},
      archivePrefix={arXiv},
      primaryClass={cs.SE}
}

@misc{zhang2023promptenhanced,
      title={Prompt-Enhanced Software Vulnerability Detection Using ChatGPT}, 
      author={Chenyuan Zhang and Hao Liu and Jiutian Zeng and Kejing Yang and Yuhong Li and Hui Li},
      year={2023},
      eprint={2308.12697},
      archivePrefix={arXiv},
      primaryClass={cs.SE}
}

@misc{sun2023gpt,
      title={When GPT Meets Program Analysis: Towards Intelligent Detection of Smart Contract Logic Vulnerabilities in GPTScan}, 
      author={Yuqiang Sun and Daoyuan Wu and Yue Xue and Han Liu and Haijun Wang and Zhengzi Xu and Xiaofei Xie and Yang Liu},
      year={2023},
      eprint={2308.03314},
      archivePrefix={arXiv},
      primaryClass={cs.CR}
}

@misc{yu2023llm,
      title={LLM for Test Script Generation and Migration: Challenges, Capabilities, and Opportunities}, 
      author={Shengcheng Yu and Chunrong Fang and Yuchen Ling and Chentian Wu and Zhenyu Chen},
      year={2023},
      eprint={2309.13574},
      archivePrefix={arXiv},
      primaryClass={cs.SE}
}

@article{li2023structured,
  title={Structured Chain-of-Thought Prompting for Code Generation},
  author={Li, Jia and Li, Ge and Li, Yongmin and Jin, Zhi},
  journal={arXiv preprint arXiv:2305.06599},
  year={2023}
}

@article{zhou2023llm,
  title={Llm as dba},
  author={Zhou, Xuanhe and Li, Guoliang and Liu, Zhiyuan},
  journal={arXiv preprint arXiv:2308.05481},
  year={2023}
}

@inproceedings{DBLP:conf/issta/WuZCK14,
  author       = {Rongxin Wu and
                  Hongyu Zhang and
                  Shing{-}Chi Cheung and
                  Sunghun Kim},
  editor       = {Corina S. Pasareanu and
                  Darko Marinov},
  title        = {CrashLocator: locating crashing faults based on crash stacks},
  booktitle    = {International Symposium on Software Testing and Analysis, {ISSTA}
                  '14, San Jose, CA, {USA} - July 21 - 26, 2014},
  pages        = {204--214},
  publisher    = {{ACM}},
  year         = {2014},
  url          = {https://doi.org/10.1145/2610384.2610386},
  doi          = {10.1145/2610384.2610386},
  timestamp    = {Mon, 03 Jan 2022 22:21:03 +0100},
  biburl       = {https://dblp.org/rec/conf/issta/WuZCK14.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/msr/WangKZ13,
  author       = {Shaohua Wang and
                  Foutse Khomh and
                  Ying Zou},
  editor       = {Thomas Zimmermann and
                  Massimiliano Di Penta and
                  Sunghun Kim},
  title        = {Improving bug localization using correlations in crash reports},
  booktitle    = {Proceedings of the 10th Working Conference on Mining Software Repositories,
                  {MSR} '13, San Francisco, CA, USA, May 18-19, 2013},
  pages        = {247--256},
  publisher    = {{IEEE} Computer Society},
  year         = {2013},
  url          = {https://doi.org/10.1109/MSR.2013.6624036},
  doi          = {10.1109/MSR.2013.6624036},
  timestamp    = {Thu, 23 Mar 2023 23:57:41 +0100},
  biburl       = {https://dblp.org/rec/conf/msr/WangKZ13.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/sigsoft/0001R18,
  author       = {Mohammad Masudur Rahman and
                  Chanchal K. Roy},
  editor       = {Gary T. Leavens and
                  Alessandro Garcia and
                  Corina S. Pasareanu},
  title        = {Improving IR-based bug localization with context-aware query reformulation},
  booktitle    = {Proceedings of the 2018 {ACM} Joint Meeting on European Software Engineering
                  Conference and Symposium on the Foundations of Software Engineering,
                  {ESEC/SIGSOFT} {FSE} 2018, Lake Buena Vista, FL, USA, November 04-09,
                  2018},
  pages        = {621--632},
  publisher    = {{ACM}},
  year         = {2018},
  url          = {https://doi.org/10.1145/3236024.3236065},
  doi          = {10.1145/3236024.3236065},
  timestamp    = {Tue, 01 Feb 2022 10:45:16 +0100},
  biburl       = {https://dblp.org/rec/conf/sigsoft/0001R18.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{DBLP:journals/smr/NayrollesHTL17,
  author       = {Mathieu Nayrolles and
                  Abdelwahab Hamou{-}Lhadj and
                  Sofi{\`{e}}ne Tahar and
                  Alf Larsson},
  title        = {A bug reproduction approach based on directed model checking and crash
                  traces},
  journal      = {J. Softw. Evol. Process.},
  volume       = {29},
  number       = {3},
  year         = {2017},
  url          = {https://doi.org/10.1002/smr.1789},
  doi          = {10.1002/smr.1789},
  timestamp    = {Mon, 26 Jun 2023 20:56:06 +0200},
  biburl       = {https://dblp.org/rec/journals/smr/NayrollesHTL17.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{DBLP:conf/icse/JinO12,
  author       = {Wei Jin and
                  Alessandro Orso},
  editor       = {Martin Glinz and
                  Gail C. Murphy and
                  Mauro Pezz{\`{e}}},
  title        = {BugRedux: Reproducing field failures for in-house debugging},
  booktitle    = {34th International Conference on Software Engineering, {ICSE} 2012,
                  June 2-9, 2012, Zurich, Switzerland},
  pages        = {474--484},
  publisher    = {{IEEE} Computer Society},
  year         = {2012},
  url          = {https://doi.org/10.1109/ICSE.2012.6227168},
  doi          = {10.1109/ICSE.2012.6227168},
  timestamp    = {Thu, 23 Mar 2023 23:58:10 +0100},
  biburl       = {https://dblp.org/rec/conf/icse/JinO12.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@misc{wu2023large,
      title={Large Language Models in Fault Localisation}, 
      author={Yonghao Wu and Zheng Li and Jie M. Zhang and Mike Papadakis and Mark Harman and Yong Liu},
      year={2023},
      eprint={2308.15276},
      archivePrefix={arXiv},
      primaryClass={cs.SE}
}

@article{Soltani2019ABE,
  title={A benchmark-based evaluation of search-based crash reproduction},
  author={Mozhan Soltani and Pouria Derakhshanfar and Xavier Devroey and Arie van Deursen},
  journal={Empirical Software Engineering},
  year={2019},
  volume={25},
  pages={138 - 96},
  url={https://api.semanticscholar.org/CorpusID:216447501}
}

@inproceedings{du2023kg4crasolver,
  title={KG4CraSolver: Recommending Crash Solutions via Knowledge Graph},
  author={Du, Xueying and Lou, Yiling and Liu, Mingwei and Peng, Xin and Yang, Tianyong},
  booktitle={Proceedings of the 31st ACM Joint European Software Engineering Conference and Symposium on the Foundations of Software Engineering},
  pages={1242--1254},
  year={2023}
}

@article{jiang2023self,
  title={Self-planning code generation with large language model},
  author={Jiang, Xue and Dong, Yihong and Wang, Lecheng and Shang, Qiwei and Li, Ge},
  journal={arXiv preprint arXiv:2303.06689},
  year={2023}
}
@misc{meta_llama_3_8b_2024,
  author    = {Meta},
  title     = {Meta-Llama-3-8B-Instruct},
  year      = {2024},
  howpublished = {\url{https://huggingface.co/meta-llama/Meta-Llama-3-8B-Instruct}},
}
@misc{gemma2024,
  author    = {Google},
  title     = {Gemma-7B-IT},
  year      = {2024},
  howpublished = {\url{https://huggingface.co/google/gemma-7b-it}},
}

@article{gao2023retrieval,
  title={Retrieval-augmented generation for large language models: A survey},
  author={Gao, Yunfan and Xiong, Yun and Gao, Xinyu and Jia, Kangxiang and Pan, Jinliu and Bi, Yuxi and Dai, Yi and Sun, Jiawei and Wang, Haofen},
  journal={arXiv preprint arXiv:2312.10997},
  year={2023}
}

@article{ahmad2021unified,
  title={Unified pre-training for program understanding and generation},
  author={Ahmad, Wasi Uddin and Chakraborty, Saikat and Ray, Baishakhi and Chang, Kai-Wei},
  journal={arXiv preprint arXiv:2103.06333},
  year={2021}
}
@article{chen2021evaluating,
  title={Evaluating large language models trained on code},
  author={Chen, Mark and Tworek, Jerry and Jun, Heewoo and Yuan, Qiming and Pinto, Henrique Ponde De Oliveira and Kaplan, Jared and Edwards, Harri and Burda, Yuri and Joseph, Nicholas and Brockman, Greg and others},
  journal={arXiv preprint arXiv:2107.03374},
  year={2021}
}
@article{rae2021scaling,
  title={Scaling language models: Methods, analysis \& insights from training gopher},
  author={Rae, Jack W and Borgeaud, Sebastian and Cai, Trevor and Millican, Katie and Hoffmann, Jordan and Song, Francis and Aslanides, John and Henderson, Sarah and Ring, Roman and Young, Susannah and others},
  journal={arXiv preprint arXiv:2112.11446},
  year={2021}
}


@article{austin2021program,
  title={Program synthesis with large language models},
  author={Austin, Jacob and Odena, Augustus and Nye, Maxwell and Bosma, Maarten and Michalewski, Henryk and Dohan, David and Jiang, Ellen and Cai, Carrie and Terry, Michael and Le, Quoc and others},
  journal={arXiv preprint arXiv:2108.07732},
  year={2021}
}
@misc{chatgpt2023,
  title        = {ChatGPT: Optimizing Language Models for Dialogue},
  author       = {{OpenAI}},
  year         = {2023},
  howpublished = {\url{https://openai.com/chatgpt}},
  note         = {Accessed: November 2, 2025.}
}
@misc{lee2022accelerating,
  title={Accelerating Onboarding},
  author={Lee, Koheun},
  year={2022}
}

@article{liu2019roberta,
  title={Roberta: A robustly optimized bert pretraining approach},
  author={Liu, Yinhan and Ott, Myle and Goyal, Naman and Du, Jingfei and Joshi, Mandar and Chen, Danqi and Levy, Omer and Lewis, Mike and Zettlemoyer, Luke and Stoyanov, Veselin},
  journal={arXiv preprint arXiv:1907.11692},
  year={2019}
}



@article{mann2020language,
  title={Language models are few-shot learners},
  author={Mann, Ben and Ryder, N and Subbiah, M and Kaplan, J and Dhariwal, P and Neelakantan, A and Shyam, P and Sastry, G and Askell, A and Agarwal, S and others},
  journal={arXiv preprint arXiv:2005.14165},
  volume={1},
  year={2020}
}

@misc{Llama2,
  author={Llama2},
  year={2023},
  url={https://ai.meta.com/research/publications/llama-2-open-foundation-and-fine-tuned-chat-models/}
}
@article{hasan2021codesc,
  title={Codesc: A large code-description parallel dataset},
  author={Hasan, Masum and Muttaqueen, Tanveer and Ishtiaq, Abdullah Al and Mehrab, Kazi Sajeed and Haque, Md Mahim Anjum and Hasan, Tahmid and Ahmad, Wasi Uddin and Iqbal, Anindya and Shahriyar, Rifat},
  journal={arXiv preprint arXiv:2105.14220},
  year={2021}
}
@misc{Llama3,
  author={Llama3},
  year={2024},
  url={https://ai.meta.com/blog/meta-llama-3/}
}
@article{hambarde2023information,
  title={Information retrieval: recent advances and beyond},
  author={Hambarde, Kailash A and Proenca, Hugo},
  journal={IEEE Access},
  year={2023},
  publisher={IEEE}
}

@online{mistral2024,
  author    = {Mistral},
  title     = {Mistral-7B-Instruct-v0.2},
  year      = {2024},
  url       = {https://huggingface.co/mistralai/Mistral-7B-Instruct-v0.2},

}
@misc{codemistral2024,
  author    = {TheBloke},
  title     = {Mistral-7B-Instruct-v0.2-code-ft-GGUF},
  year      = {2024},
  howpublished = {\url{https://huggingface.co/TheBloke/Mistral-7B-Instruct-v0.2-code-ft-GGUF}},

}


@article{watson2022systematic,
  title={A systematic literature review on the use of deep learning in software engineering research},
  author={Watson, Cody and Cooper, Nathan and Palacio, David Nader and Moran, Kevin and Poshyvanyk, Denys},
  journal={ACM Transactions on Software Engineering and Methodology (TOSEM)},
  volume={31},
  number={2},
  pages={1--58},
  year={2022},
  publisher={ACM New York, NY}
}
@misc{llama2024,
  author       = {Meta},
  title        = {Llama-2-7B-HF},
  year         = {2024},
  howpublished = {\url{https://huggingface.co/meta-llama/Llama-2-7b-hf}},
  note         = {Accessed: November 2, 2025}
}


@misc{deepseek2024,
  author    = {DeepSeek-AI},
  title     = {DeepSeek-LLM-7B-Chat},
  year      = {2024},
  howpublished = {\url{https://huggingface.co/deepseek-ai/deepseek-llm-7b-chat}},
}

@misc{deepseek_coder_2024,
  author    = {DeepSeek-AI},
  title     = {DeepSeek-Coder-6.7B-Instruct},
  year      = {2024},
  howpublished = {\url{https://huggingface.co/deepseek-ai/deepseek-coder-6.7b-instruct}},

}

@misc{codegemma2024,
  author    = {Google},
  title     = {CodeGemma-7B-IT},
  year      = {2024},
  howpublished = {\url{https://huggingface.co/google/codegemma-7b-it}},

}

@misc{unixcoder2024,
  author    = {Microsoft},
  title     = {UnixCoder-Base},
  year      = {2024},
  howpublished = {\url{https://huggingface.co/microsoft/unixcoder-base}},
  
}

@misc{codebert2024,
  author    = {Microsoft},
  title     = {CodeBERT-Base},
  year      = {2024},
  howpublished = {\url{https://huggingface.co/microsoft/codebert-base}},
  
}





@misc{dubey2024llama3herdmodels,
  title = {The Llama 3 Herd of Models},
  author = {Abhimanyu Dubey and Abhinav Jauhri and Abhinav Pandey and et al.},
  year = {2024},
  eprint = {2407.21783},
  archivePrefix = {arXiv},
  primaryClass = {cs.AI},
  url = {https://arxiv.org/abs/2407.21783},
}



@article{team2024gemma,
  title={Gemma: Open models based on gemini research and technology},
  author={Team, Gemma and Mesnard, Thomas and Hardin, Cassidy and Dadashi, Robert and Bhupatiraju, Surya and Pathak, Shreya and Sifre, Laurent and Rivi{\`e}re, Morgane and Kale, Mihir Sanjay and Love, Juliette and others},
  journal={arXiv preprint arXiv:2403.08295},
  year={2024}
}
@misc{ajibawa2023code,
  author = {Ajibawa, (2023)},
  title = {Code-290k-ShareGPT},
  year = {2024},
  howpublished = {\url{https://huggingface.co/datasets/ajibawa-2023/Code-290k-ShareGPT}}
}
@article{touvron2023llama2,
  title={Llama 2: Open foundation and fine-tuned chat models},
  author={Touvron, Hugo and Martin, Louis and Stone, Kevin and Albert, Peter and Almahairi, Amjad and Babaei, Yasmine and Bashlykov, Nikolay and Batra, Soumya and Bhargava, Prajjwal and Bhosale, Shruti and others},
  journal={arXiv preprint arXiv:2307.09288},
  year={2023}
}
@article{jiang2023mistral,
  title={Mistral 7B},
  author={Jiang, Albert Q and Sablayrolles, Alexandre and Mensch, Arthur and Bamford, Chris and Chaplot, Devendra Singh and Casas, Diego de las and Bressand, Florian and Lengyel, Gianna and Lample, Guillaume and Saulnier, Lucile and others},
  journal={arXiv preprint arXiv:2310.06825},
  year={2023}
}
@article{bi2024deepseek,
  title={Deepseek llm: Scaling open-source language models with longtermism},
  author={Bi, Xiao and Chen, Deli and Chen, Guanting and Chen, Shanhuang and Dai, Damai and Deng, Chengqi and Ding, Honghui and Dong, Kai and Du, Qiushi and Fu, Zhe and others},
  journal={arXiv preprint arXiv:2401.02954},
  year={2024}
}
@article{guo2024deepseek,
  title={DeepSeek-Coder: When the Large Language Model Meets Programming--The Rise of Code Intelligence},
  author={Guo, Daya and Zhu, Qihao and Yang, Dejian and Xie, Zhenda and Dong, Kai and Zhang, Wentao and Chen, Guanting and Bi, Xiao and Wu, Yu and Li, YK and others},
  journal={arXiv preprint arXiv:2401.14196},
  year={2024}
}

@inproceedings{voorhees1999trec,
  title={The trec-8 question answering track report.},
  author={Voorhees, Ellen M and others},
  booktitle={Trec},
  volume={99},
  pages={77--82},
  year={1999}
}

@article{Bi2024DeepSeekLS,
  title={DeepSeek LLM: Scaling Open-Source Language Models with Longtermism},
  author={DeepSeek-AI Xiao Bi and Deli Chen and Guanting Chen et al.},
  journal={ArXiv},
  year={2024},
  volume={abs/2401.02954},
  url={https://doi.org/10.48550/arXiv.2401.02954},
}

@misc{Gemmma,
  author={Gemma},
  year={2024},
  url={https://blog.google/technology/developers/gemma-open-models/}
}


@misc{Code-Mistral,
  author={Code-Mistral},
  year={2024},
  url={https://huggingface.co/ajibawa-2023/Code-Mistral-7B}
}

@misc{deepseek-coder,
  title = {DeepSeek-Coder: When the Large Language Model Meets Programming -- The Rise of Code Intelligence},
  author = {Daya Guo and Qihao Zhu and Dejian Yang et al.},
  journal = {CoRR},
  volume = {abs/2401.14196},
  year = {2024},
  url = {https://arxiv.org/abs/2401.14196}
}

@article{Zhao2024CodeGemmaOC,
  title={CodeGemma: Open Code Models Based on Gemma},
  author={CodeGemma Team Heri Zhao and Jeffrey Hui and Joshua Howland and Nam Nguyen and Siqi Zuo and Andrea Hu and Christopher A. Choquette-Choo and Jingyue Shen and Joe Kelley and Kshitij Bansal and Luke Vilnis and Mateo Wirth and Paul Michel and Peter Choy and Pratik Joshi and Ravin Kumar and Sarmad Hashmi and Shubham Agrawal and Zhitao Gong and Jane Fine and Tris Brian Warkentin and Ale Jakse Hartman and Bin Ni and Kathy Korevec and Kelly Schaefer and Scott Huffman},
  journal={ArXiv},
  year={2024},
  volume={abs/2406.11409},
  url={https://doi.org/10.48550/arXiv.2406.11409}
}

@article{Rozire2023CodeLO,
  title={Code Llama: Open Foundation Models for Code},
  author={Baptiste Rozi{\`e}re and Jonas Gehring and Fabian Gloeckle and Sten Sootla and Itai Gat and Xiaoqing Tan and Yossi Adi and Jingyu Liu and Tal Remez and J{\'e}r{\'e}my Rapin and Artyom Kozhevnikov and I. Evtimov and Joanna Bitton and Manish P Bhatt and Cristian Cant{\'o}n Ferrer and Aaron Grattafiori and Wenhan Xiong and Alexandre D'efossez and Jade Copet and Faisal Azhar and Hugo Touvron and Louis Martin and Nicolas Usunier and Thomas Scialom and Gabriel Synnaeve},
  journal={ArXiv},
  year={2023},
  volume={abs/2308.12950},
  url={https://doi.org/10.48550/arXiv.2308.12950}
}


@inproceedings{chatterjee2009sniff,
  title={Sniff: A search engine for java using free-form queries},
  author={Chatterjee, Shaunak and Juvekar, Sudeep and Sen, Koushik},
  booktitle={Fundamental Approaches to Software Engineering: 12th International Conference, FASE 2009, Held as Part of the Joint European Conferences on Theory and Practice of Software, ETAPS 2009, York, UK, March 22-29, 2009. Proceedings 12},
  pages={385--400},
  year={2009},
  organization={Springer}
}

@inproceedings{mcmillan2011portfolio,
  title={Portfolio: finding relevant functions and their usage},
  author={McMillan, Collin and Grechanik, Mark and Poshyvanyk, Denys and Xie, Qing and Fu, Chen},
  booktitle={Proceedings of the 33rd International Conference on Software Engineering},
  pages={111--120},
  year={2011}
}
@article{nie2016query,
  title={Query expansion based on crowd knowledge for code search},
  author={Nie, Liming and Jiang, He and Ren, Zhilei and Sun, Zeyi and Li, Xiaochen},
  journal={IEEE Transactions on Services Computing},
  volume={9},
  number={5},
  pages={771--783},
  year={2016},
  publisher={IEEE}
}
@article{feng2020codebert,
  title={Codebert: A pre-trained model for programming and natural languages},
  author={Feng, Zhangyin and Guo, Daya and Tang, Duyu and Duan, Nan and Feng, Xiaocheng and Gong, Ming and Shou, Linjun and Qin, Bing and Liu, Ting and Jiang, Daxin and others},
  journal={arXiv preprint arXiv:2002.08155},
  year={2020}
}
@article{guo2020graphcodebert,
  title={Graphcodebert: Pre-training code representations with data flow},
  author={Guo, Daya and Ren, Shuo and Lu, Shuai and Feng, Zhangyin and Tang, Duyu and Liu, Shujie and Zhou, Long and Duan, Nan and Svyatkovskiy, Alexey and Fu, Shengyu and others},
  journal={arXiv preprint arXiv:2009.08366},
  year={2020}
}
@article{devlin2018bert,
  title={Bert: Pre-training of deep bidirectional transformers for language understanding},
  author={Devlin, Jacob and Chang, Ming-Wei and Lee, Kenton and Toutanova, Kristina},
  journal={arXiv preprint arXiv:1810.04805},
  year={2018}
}
@article{guo2022unixcoder,
  title={Unixcoder: Unified cross-modal pre-training for code representation},
  author={Guo, Daya and Lu, Shuai and Duan, Nan and Wang, Yanlin and Zhou, Ming and Yin, Jian},
  journal={arXiv preprint arXiv:2203.03850},
  year={2022}
}
@article{wang2021codet5,
  title={Codet5: Identifier-aware unified pre-trained encoder-decoder models for code understanding and generation},
  author={Wang, Yue and Wang, Weishi and Joty, Shafiq and Hoi, Steven CH},
  journal={arXiv preprint arXiv:2109.00859},
  year={2021}
}
@article{wang2023codet5+,
  title={Codet5+: Open code large language models for code understanding and generation},
  author={Wang, Yue and Le, Hung and Gotmare, Akhilesh Deepak and Bui, Nghi DQ and Li, Junnan and Hoi, Steven CH},
  journal={arXiv preprint arXiv:2305.07922},
  year={2023}
}
@article{T5,
  title={Exploring the limits of transfer learning with a unified text-to-text transformer},
  author={Raffel, Colin and Shazeer, Noam and Roberts, Adam and Lee, Katherine and Narang, Sharan and Matena, Michael and Zhou, Yanqi and Li, Wei and Liu, Peter J},
  journal={Journal of machine learning research},
  volume={21},
  number={140},
  pages={1--67},
  year={2020}
}
@article{gpt4,
  title={Gpt-4 technical report},
  author={Achiam, Josh and Adler, Steven and Agarwal, Sandhini and Ahmad, Lama and Akkaya, Ilge and Aleman, Florencia Leoni and Almeida, Diogo and Altenschmidt, Janko and Altman, Sam and Anadkat, Shyamal and others},
  journal={arXiv preprint arXiv:2303.08774},
  year={2023}
}

==> sections/RQ3/RQ3_design.tex <==

\subsection{Design}
\label{sec:rq3-design}




==> sections/abstract.tex <==
Code search is crucial for code reuse, enabling developers to efficiently locate relevant snippets. Current methods rely on encoder-based models, which suffer from limitations such as poor generalization and restricted input lengths. Decoder-only large language models (LLMs), with their extensive pre-training, larger size, and longer input capabilities, offer potential solutions to these issues, yet their effectiveness in code search remains underexplored.

To fill this gap, our study presents the first systematic exploration of decoder-only LLMs for code search.
We evaluate nine state-of-the-art decoder-only models using two fine-tuning methods, two datasets (CSN and CoSQA$^+$), and three model sizes. Our findings reveal that fine-tuned CodeGemma significantly outperforms encoder-only models like UniXcoder, achieving a 5.57\% improvement in MRR on CSN and a 49.6\% increase in MAP on CoSQA$^+$ compared to zero-shot UniXcoder. These results highlight the superior performance and adaptability of decoder-only models. Additionally, we provide valuable insights into optimizing these models for code search, covering aspects such as model selection, fine-tuning methods, training data, and model size, and discussing their strengths and limitations.






















==> tables/finetune.tex <==
\begin{table*}[h!] 
  \centering
  \caption{Finetuned result on code search benchmarks.}


    \begin{tabular}{|p{5.555em}|c|c|c|c|c|c|c|c|c|}
    \toprule
    \multicolumn{1}{|r|}{} & \multicolumn{7}{c|}{CSN(MRR)}                         & \multicolumn{2}{c|}{CoSQA+} \\
    \midrule
    \multicolumn{1}{|c|}{Sup Model} & Ruby  & Javascript & Go    & Python & Java  & Php   & Avg.  & MAP   & MRR \\
    \midrule
    Codebert &       &       &       &       &       &       &       &       &  \\
    \midrule
    UnixCode & 0.592  & 0.581  & 0.667  & 0.760  & 0.719  & 0.691  & 0.701  & 0.02585  & 0.03070  \\
    \midrule
    CodeGemma & \textbf{0.662 } & \textbf{0.643 } & 0.786  & \textbf{0.776 } & \textbf{0.749 } & \textbf{0.709 } & \textbf{0.740 } & 0.24168  & \textbf{0.28357 } \\
    \midrule
    Gemma & 0.642  & 0.614  & \textbf{0.799 } & 0.741  & 0.736  & 0.698  & 0.725  & 0.24592  & 0.28577  \\
    \midrule
    DeepseekCoder & 0.608  & 0.639  & 0.708  & 0.752  & 0.741  & 0.723  & 0.724  & 0.14260  & 0.17523  \\
    \midrule
    DeepseekLlm & 0.610  & 0.608  & 0.744  & 0.719  & 0.742  & 0.720  & 0.719  & 0.01001  & 0.01132  \\
    \midrule
    Llama3 & 0.550  & 0.579  & 0.733  & 0.718  & 0.709  & 0.681  & 0.694  & 0.19349  & 0.24008  \\
    \midrule
    CodeMistral & \multicolumn{1}{p{4.555em}|}{x} & \multicolumn{1}{p{4.555em}|}{x} & \multicolumn{1}{p{4.555em}|}{x} &       &       &       &       & \multicolumn{1}{p{4.555em}|}{x} & \multicolumn{1}{p{4.555em}|}{x} \\
    \midrule
    Mistral & 0.562  & 0.571  & 0.732  & 0.684  & 0.722  & 0.686  & 0.692  & \textbf{0.28357 } & 0.24168  \\
    \midrule
    CodeLlama & 0.415  & 0.515  & 0.549  & 0.578  & 0.634  & 0.564  & 0.577  & \multicolumn{1}{p{4.555em}|}{x} & \multicolumn{1}{p{4.555em}|}{x} \\
    \midrule
    Llama2 & 0.392  & 0.471  & 0.584  & 0.568  & 0.580  & 0.503  & 0.545  & 0.01592  & 0.01911  \\



    \bottomrule
    \end{tabular}%
  \label{tab:finetune_result}%
\end{table*}%
